GANav: Efficient Terrain Segmentation for Robot Navigation in Unstructured Outdoor Environments

We propose GANav, a novel group-wise attention mechanism to identify safe and navigable regions in off-road terrains and unstructured environments from RGB images. Our approach classifies terrains based on their navigability levels using coarse-grained semantic segmentation. Our novel group-wise attention loss enables any backbone network to explicitly focus on the different groups' features with low spatial resolution. Our design leads to efficient inference while maintaining a high level of accuracy compared to existing SOTA methods. Our extensive evaluations on the RUGD and RELLIS-3D datasets shows that GANav achieves an improvement over the SOTA mIoU by 2.25-39.05% on RUGD and 5.17-19.06% on RELLIS-3D. We interface GANav with a deep reinforcement learning-based navigation algorithm and highlight its benefits in terms of navigation in real-world unstructured terrains. We integrate our GANav-based navigation algorithm with ClearPath Jackal and Husky robots, and observe an increase of 10% in terms of success rate, 2-47% in terms of selecting the surface with the best navigability and a decrease of 4.6-13.9% in trajectory roughness. Further, GANav reduces the false positive rate of forbidden regions by 37.79%. Code, videos, and a full technical report are available at https://gamma.umd.edu/offroad/.

==> QualitativeResults/qualitative.tex <==

% \begin{figure*}[t]
%     \centering
%     %\captionsetup[subfigure]{labelformat=empty}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set2/img.png}
%     \caption{Image}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set2/gtgroup.png}
%     \caption{GT}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set2/pred_psp.png}
%     \caption{PSPNet~\cite{zhao2017pyramid}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set2/pred_ocr.png}
%     \caption{OCRNet~\cite{yuan2020objectcontextual}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set2/pred_ours.png}
%     \caption{Ours}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set3/img.png}
%     \caption{Image}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set3/gtgroup.png}
%     \caption{GT}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set3/pred_psp.png}
%     \caption{PSPNet~\cite{zhao2017pyramid}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set3/pred_ocr.png}
%     \caption{OCRNet~\cite{yuan2020objectcontextual}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set3/pred_ours.png}
%     \caption{Ours}
%     \end{subfigure}   
%     % \\
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set4/img.png}
%     % \caption{Image}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set4/gtgroup.png}
%     % \caption{GT}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set4/pred_psp.png}
%     % \caption{PSPNet}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set4/pred_ocr.png}
%     % \caption{OCRNet}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set4/pred_ours.png}
%     % \caption{Ours}
%     % \end{subfigure}
%     % \\        
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set5/img.png}
%     % \caption{Image}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set5/gtgroup.png}
%     % \caption{GT}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set5/pred_psp.png}
%     % \caption{PSPNet}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set5/pred_ocr.png}
%     % \caption{OCRNet}
%     % \end{subfigure}
%     % \begin{subfigure}[b]{0.18\textwidth}
%     % \includegraphics[width = \textwidth]{QualitativeResults/set5/pred_ours.png}
%     % \caption{Ours}
%     % \end{subfigure}
%     \\      
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set6/img.png}
%     \caption{Image}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set6/gtgroup.png}
%     \caption{GT}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set6/pred_psp.png}
%     \caption{PSPNet~\cite{zhao2017pyramid}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set6/pred_ocr.png}
%     \caption{OCRNet~\cite{yuan2020objectcontextual}}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.18\textwidth}
%     \includegraphics[width = \textwidth]{QualitativeResults/set6/pred_ours.png}
%     \caption{Ours}
%     \end{subfigure}
%     \\      
%     % \begin{subfigure}[c]{0.49\textwidth}
%     % \includegraphics[width = \textwidth]{fig/legend1.png}
%     % \end{subfigure}
%     % \begin{subfigure}[c]{0.49\textwidth}
%     % \includegraphics[width = \textwidth]{fig/legend2.png}
%     % \end{subfigure}
%     \begin{subfigure}[c]{0.95\textwidth}
%     \includegraphics[width = \textwidth]{fig/legend.png}
%     \end{subfigure}


    
    
%     % \caption{\textbf{Qualitative Results:} Write more \rohan{Just Marking this so that we remember to edit it.}}
%     \caption{\textbf{Qualitative Results:} Each row highlights  the original image, ground truth (GT) label, prediction of two SOTA methods and prediction of our method. We observe that our method is able to detect different navigable regions and is robust with respect to objects with similar color, as shown in image (k).}
%     \label{fig:visualisations}
%     \vspace{-3mm}

% \end{figure*}


\begin{figure*}[t]
    \centering

    \begin{subfigure}[c]{0.95\textwidth}
    \includegraphics[width = \textwidth]{fig/world2.png}
    \end{subfigure}
    \\      
    % \begin{subfigure}[c]{0.49\textwidth}
    % \includegraphics[width = \textwidth]{fig/legend1.png}
    % \end{subfigure}
    % \begin{subfigure}[c]{0.49\textwidth}
    % \includegraphics[width = \textwidth]{fig/legend2.png}
    % \end{subfigure}
    \begin{subfigure}[c]{0.95\textwidth}
    \includegraphics[width = \textwidth]{fig/legend.png}
    \end{subfigure}


    
    
    % \caption{\textbf{Qualitative Results:} Write more \rohan{Just Marking this so that we remember to edit it.}}
    \caption{\textbf{Qualitative results in the wild:} We show the real-world performance of \ours{} and two SOTA methods with pre-trained models on RUGD and RELLIS-3D. The green trajectory is the path of the robot in the next 2 seconds based on its current velocity. While other methods have some false positives on the forbidden region and over-generalize on the rough region (in yellow), our method can correctly identify different regions and stay on the safest path.}
    \label{fig:realworld}
    \vspace{-3mm}

\end{figure*}



==> Tables/ablation.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
  \toprule
\textbf{Backbone} & \textbf{GW-Attn.}   & \textbf{mIoU} $\uparrow$ & \textbf{mAcc} $\uparrow$ & \textbf{aAcc} $\uparrow$ \\
  \midrule
% \hline
\multirow{1}[3]{*}{ResNet50~\cite{resnet}} & \ding{55} & 71.55 & 87.67  & 91.63 \\ 
  & \checkmark & 78.22  & 85.09 & 92.91 \\ 
  \midrule
 \multirow{1}[3]{*}{BoT~\cite{srinivas2021bottleneck}}   & \ding{55}  & 74.32 & 80.41 & 93.53 \\ 
  & \checkmark & 83.24 & 89.84 & 94.26 \\ 
  \midrule
  \multirow{1}[3]{*}{MiT~\cite{segformer}}   & \ding{55}  & 77.64 & 86.78 & 93.47  \\ 
  & \checkmark & 89.08  & 93.55 & 95.66 \\ 
%   \midrule
%   \multirow{5}[6]{*}{RELLIS-3D} & \multirow{1}[3]{*}{ResNet50\cite{resnet}}  &  & 61.82  & 71.55 & 81.72 \\ 
%     &&    \checkmark & 63.31 & 71.57 & 83.14\\ 
%              \cmidrule{2-6}
%       &  \multirow{1}[3]{*}{BoT~\cite{srinivas2021bottleneck}} && 63.01 & 68.7 & 92.2 \\ 
%     &&  \checkmark & 70.63 & 81.32 & 90.23\\ 
%              \cmidrule{2-6}
%       &  \multirow{1}[3]{*}{MiT~\cite{segformer}}  & & 68.91 & 81.5 & 85.57 \\ 
%     &&    \checkmark & 74.44 & 86.49 & 91.69\\ 
  \bottomrule
\end{tabular}
}
\caption{\textbf{Ablation studies on GA heads with different backbones on RUGD val sets:} We observe that the group-wise attention mechanism is successful in improving mIoU by \rt{at least $7.26\%$}, regardless of the backbone choice.
% Dynamic class weighting (DW) leads to better performance on RELLIS-3D, which have lower mIoU and accuracy. We didn't get much improvement on RUGD with DW since the accuracy is saturated.
}

% \caption{Ablation studies on the RUGD and RELLIS-3D val sets. We observe that the group-wise attention mechanism is successful in improving mIoU by $7.26-11.44\%$ and $4.18-10.31\%$ on the RUGD and RELLIS datasets, respectively, regardless of the backbone choice.
% % Dynamic class weighting (DW) leads to better performance on RELLIS-3D, which have lower mIoU and accuracy. We didn't get much improvement on RUGD with DW since the accuracy is saturated.
% }

\label{tab:ablation}

\vspace{-7mm}
\end{table}








% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lc|ccccc}
%   \toprule
%   \multicolumn{2}{c}{Dataset} & Backbone & GW-Attn.   & mIoU & mAcc & aAcc \\
%   \midrule
%   \multicolumn{2}{c}{\multirow{4}[6]{*}{RUGD}} & \multirow{1}[3]{*}{xxx} &  & 74.32 & 80.41 & 93.53 \\ 
%   &&& \checkmark & 83.24 & 89.84 & 94.26 \\ 
  
% & & \multirow{1}[3]{*}{xxx}   &   & 74.32 & 80.41 & 93.53 \\ 
%   &&& \checkmark & 83.24 & 89.84 & 94.26 \\ 
  
% & & \multirow{1}[3]{*}{xxx}   &   & 74.32 & 80.41 & 93.53 \\ 
%   &&& \checkmark & 83.24 & 89.84 & 94.26 \\ 
%   \midrule
%   \multicolumn{2}{c}{\multirow{4}[6]{*}{RELLIS-3D}} & \multirow{1}[3]{*}{xxx}  &  & 63.01 & 68.7 & 92.2 \\ 
%     &&&    \checkmark & 70.63 & 81.32 & 90.23\\ 
    
%       & & \multirow{1}[3]{*}{xxx} && 63.01 & 68.7 & 92.2 \\ 
%     && & \checkmark & 70.63 & 81.32 & 90.23\\ 
    
%       & & \multirow{1}[3]{*}{xxx}   & & 63.01 & 68.7 & 92.2 \\ 
%     &&   & \checkmark & 70.63 & 81.32 & 90.23\\ 
%   \bottomrule
% \end{tabular}
% }
% \caption{Ablation studies on the RUGD and RELLIS-3D test sets. We observe that the group-wise attention mechanism is successful in improving mIoU by $8.68\%$ and $7.62\%$ on the RUGD and RELLIS datasets, respectively.
% % Dynamic class weighting (DW) leads to better performance on RELLIS-3D, which have lower mIoU and accuracy. We didn't get much improvement on RUGD with DW since the accuracy is saturated.
% }

% \label{tab:ablation}

% \vspace{-2mm}
% \end{table}

==> Tables/ablation2.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
  \toprule
\textbf{Spatial Reduction} & \textbf{GW-Attn.}   & \textbf{mIoU} $\uparrow$ & \textbf{mAcc} $\uparrow$ & \textbf{aAcc} $\uparrow$ \\
%   \midrule
%   \multirow{5}[6]{*}{RUGD} & \multirow{1}[3]{*}{\large{$\frac{1}{8} \times \frac{1}{8}$}} &  & 77.64 & 86.78  & 93.47 \\ 
%   && \checkmark & 89.08 & 93.55 & 95.66 \\ 
%          \cmidrule{2-6}
% &  \multirow{1}[3]{*}{\large{$\frac{1}{16} \times \frac{1}{16}$}}   &   & 79.61 & 87.76 & 92.85 \\ 
%   && \checkmark & 87.07 & 91.74 & 94.99 \\ 
%           \cmidrule{2-6}
% &  \multirow{1}[3]{*}{\large{$\frac{1}{32} \times \frac{1}{32}$}}   &   & 76.81 & 85.14 & 92.24  \\ 
%   && \checkmark & 84.9  & 90.36 & 94.24 \\ 
  \midrule
 \multirow{1}[3]{*}{\large{$\frac{1}{8} \times \frac{1}{8}$}}  & \ding{55} & 68.91  & 81.5 & 85.57 \\ 
    &    \checkmark & 71.76 & 81.62 & 90.31\\ 
  \midrule
         \multirow{1}[3]{*}{\large{$\frac{1}{16} \times \frac{1}{16}$}} & \ding{55} & 67.61 & 79.95 & 84.03 \\ 
    &  \checkmark & 71.62 & 84.51 & 90.26\\ 
  \midrule
         \multirow{1}[3]{*}{\large{$\frac{1}{32} \times \frac{1}{32}$}}  & \ding{55} & 64.91 & 75.56 & 83.51 \\ 
   &    \checkmark & 70.76 & 84.4 & 90.44\\ 
  \bottomrule
\end{tabular}
}
\caption{\textbf{Ablation studies on GA heads with different spatial reduction on RELLIS-3D val sets:} We show that higher spatial reduction can decrease the perception accuracy and the group-wise attention can mitigate the performance drop due to resolution reduction. ``$\frac{1}{N}\times \frac{1}{N}$" in the second column means the bottleneck spatial resolution is reduced by a factor of N on height and width compared to the input resolution.}


\label{tab:ablation2}

\vspace{-8mm}
\end{table}








==> Tables/comparison.tex <==
% \begin{table*}[t]
% \centering
% \vspace{7pt}
% % \setlength{\tabcolsep}{2mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{l|l|cccccc|cc}
%   \toprule[2pt]
%   \textbf{Dataset} &
%   \textbf{Methods (IoU)} & \textbf{Smooth Region} & \textbf{Rough Region} & \textbf{Bumpy Region} &  \textbf{Forbidden Region} & \textbf{Obstacle} & \textbf{Background} & \textbf{mIoU} $\uparrow$ & \textbf{aAcc} $\uparrow$\\
% %   \midrule
% \hline
%      \multirow{13}[6]{*}{RUGD} & PSPNet \cite{zhao2017pyramid} & 48.62 & 88.92 & 69.45 & 29.07 & 87.98 & 78.29 & 67.06 & 92.85 \\
%      & DeepLabv3+ \cite{deeplabv3+} & 5.86 & 84.99 & 50.40 & 25.04 & 87.50 & \underline{\textbf{81.47}} & 55.88 & 91.51\\
%      & DANet \cite{fu2019dual} & 2.26 & 81.47 & 8.69 & 15.00 & 82.54 & 74.86 & 44.14 & 88.81 \\
%      & OCRNet \cite{yuan2020objectcontextual} & 66.29 & 89.47 & 76.15 & 59.14 & 88.77 & \underline{79.17} & 76.50 & 93.46 \\
%      & PSANet \cite{2018psanet} & 34.92 & 87.70 & 35.64 & 8.66 & 86.95 & 78.97 & 55.47 & 92.13 \\
     
%      & BiseNetv2~\cite{bisenetv2} & 24.27 & 89.99 & \underline{\textbf{89.99}} & 83.31 & 90.93 & 75.29 & 75.1 & 93.4  \\
%      & CGNet~\cite{cgnet} & 40.84 & 90.39 & 85.67 & 76.21 & 89.75 & 74.48 & 76.22 & 93.29  \\
%      & FastSCNN~\cite{fastscnn} & 83.03 & 92.82 & 87.69 & 81.05 & 90.94 & 75.11 & 85.11 & 94.77 \\
%      & FastFCN~\cite{fastfcn}  & 26.27 & 89.85 & 85.95 & \underline{84.13} & \underline{91.23} & 75.63 & 75.51 & 93.46 \\
%     %   \cmidrule(lr{1em}){2-9}
%       \cmidrule{2-10}
%      & *SETR~\cite{setr} & 89.77 & 92.46 & 84.58 & 70.33 & 89.55 & 70.47 & 82.86 & 94.09 \\
%      & *DPT~\cite{dpt} & 1.04 & 81.23 & 22.98 & 25.84 & 89.18 & 74.5 & 49.13 & 88.77 \\
%      & *Segformer~\cite{segformer} & \underline{93.26} & \underline{93.16} & 87.56 & 77.31 & 91.2 & 78.5 & \underline{86.83} & \underline{95.17}  \\
%      & *Segmenter~\cite{segmenter} & 90.39 & 91.17 & 83.96 & 65.43 & 87.8 & 68.17 & 81.15 & 93.22  \\
%      & \textbf{*\ours\ (ours)} & \underline{\textbf{94.61}} & \underline{\textbf{93.71}} & \underline{89.69} & \underline{\textbf{85.43}} & \underline{\textbf{91.41}} & 76.11 & \underline{\textbf{88.49}} & \underline{\textbf{95.33}}  \\

% %   \midrule
%   \midrule
% % \cmidrule{1-9}
%      \multirow{13}[6]{*}{RELLIS-3D} & PSPNet \cite{zhao2017pyramid} & 69.21 & 80.99 & 8.89 & 53.7 & 60.7 & 94.67 & 61.36 & 86.01 \\
%      & DeepLabv3+ \cite{deeplabv3+} & 65.76 & 79.84 & 19.72 & 47.52 & 64.88 & \underline{95.92} & 62.27 & 85.84\\
%      & DANet \cite{fu2019dual} & 72.93 & \underline{85.18} & 13.10 & \underline{60.60} & 70.53 & \underline{\textbf{95.95}} & 66.38 & \underline{89.11}\\
%      & OCRNet \cite{yuan2020objectcontextual} & \underline{74.67} & 83.04 & 27.76 & 60.44 & 62.35 & 92.58 & 66.81 & 86.95\\
%      & PSANet \cite{2018psanet} & 64.06 & 75.29 & 17.08 & 47.45 & 61.74 & 94.31 & 59.99 & 83.17 \\
     
%      & BiseNetv2~\cite{bisenetv2} & 65.56 & 73.24 & 39.35 & 48.17 & \underline{\textbf{71.91}} & 93.78 & 65.33 & 83.03    \\
%      & CGNet~\cite{cgnet} & 62.84 & 74.17 & 49.57 & 45.41 & 68.88 & 94.53 & 65.9 & 82.7 \\
%      & FastSCNN~\cite{fastscnn} & 67.06 & 77.6 & \underline{\textbf{56.49}} & 49.76 & 70.31 & 94.43 & \underline{69.27} & 84.51 \\
%      & FastFCN~\cite{fastfcn} & 70.51 & 79.15 & \underline{49.72} & 51.37 & 63.9 & 94.82 & 68.24 & 84.1 \\            \cmidrule{2-10}

%      & *SETR~\cite{setr} & 65.37 & 78.64 & 40.89 & 52.59 & 63.8 & 91.87 & 65.53 & 83.59 \\
%      & *DPT~\cite{dpt} & 5.42 & 76.65 & 47.13 & 54.87 & 62.74 & 85.5 & 55.38 & 81.61 \\
%      & *Segformer~\cite{segformer} & 60.28 & 79.78 & 53.35 & 53.78 & 70.15 & 94.37 & 68.62 & 85.37\\
%      & *Segmenter~\cite{segmenter} & 51.67 & 78.4 & 19.38 & 42.61 & 66.04 & 92.05 & 58.36 & 82.16\\
%      & \textbf{*\ours\ (ours)} & \underline{\textbf{78.5}} & \underline{\textbf{85.78}} & 31.68 & \underline{\textbf{67.05}} & \underline{71.67} & 95.87 & \underline{\textbf{71.76}} & \underline{\textbf{90.31}}  \\

%   \bottomrule[2 pt]
% %   \bottomrule
% \end{tabular}

% \end{adjustbox}
% \caption{\textbf{Comparison with state-of-the-art methods on RUGD and RELLIS-3D val sets:} We compare the performance of our learning method with transformer-based methods (with *) as well as other methods in terms of IoU.  Our \ours{} method improves the state-of-the-art mIoU by $1.66-44.35\%$ on RUGD and $2.49-16.38\%$ on RELLIS-3D. Further, we show that our grouping method can improve the accuracy of classes like smooth region, bumpy region, and forbidden regions by large margins, thus improving safe navigation. We underscore the best and second-best results and bold the best number.}
% % \vspace{-5mm}
% \label{tab:comparison}
% \end{table*}



\begin{table*}[t]
\centering
\vspace{7pt}
% \setlength{\tabcolsep}{2mm}
\ra{1.05}
\Large
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|l|cccccc|cc}
  \toprule[2pt]
  \textbf{Dataset} &
  \textbf{Methods (IoU)} & \textbf{Smooth Region} & \textbf{Rough Region} & \textbf{Bumpy Region} &  \textbf{Forbidden Region} & \textbf{Obstacle} & \textbf{Background} & \textbf{mIoU} $\uparrow$ & \textbf{aAcc} $\uparrow$\\
%   \midrule
\hline
     \multirow{11}[5]{*}{RUGD} & PSPNet \cite{zhao2017pyramid} & 48.62 & 88.92 & 69.45 & 29.07 & 87.98 & 78.29 & 67.06 & 92.85 \\
    %  & DeepLabv3+ \cite{deeplabv3+} & 5.86 & 84.99 & 50.40 & 25.04 & 87.50 & \underline{\textbf{81.47}} & 55.88 & 91.51\\
    %  & DANet \cite{fu2019dual} & 2.26 & 81.47 & 8.69 & 15.00 & 82.54 & 74.86 & 44.14 & 88.81 \\
     & OCRNet \cite{yuan2020objectcontextual} & 66.29 & 89.47 & 76.15 & 59.14 & 88.77 & \underline{\textbf{79.17}} & 76.50 & 93.46 \\
    %  & PSANet \cite{2018psanet} & 34.92 & 87.70 & 35.64 & 8.66 & 86.95 & 78.97 & 55.47 & 92.13 \\
     
    %  & BiseNetv2~\cite{bisenetv2} & 24.27 & 89.99 & \underline{\textbf{89.99}} & 83.31 & 90.93 & 75.29 & 75.1 & 93.4  \\
     & CGNet~\cite{cgnet} & 40.84 & 90.39 & 85.67 & 76.21 & 89.75 & 74.48 & 76.22 & 93.29  \\
     & FastSCNN~\cite{fastscnn} & 83.03 & 92.82 & \underline{87.69} & \underline{81.05} & 90.94 & 75.11 & 85.11 & 94.77 \\
    %  & FastFCN~\cite{fastfcn}  & 26.27 & 89.85 & 85.95 & \underline{84.13} & \underline{91.23} & 75.63 & 75.51 & 93.46 \\
    %   \cmidrule(lr{1em}){2-9}
        %   \cmidrule{2-10}
     & *SETR~\cite{setr} & 89.77 & 92.46 & 84.58 & 70.33 & 89.55 & 70.47 & 82.86 & 94.09 \\
     & *DPT~\cite{dpt} & 1.04 & 81.23 & 22.98 & 25.84 & 89.18 & 74.5 & 49.13 & 88.77 \\
     & *Segformer~\cite{segformer} & \underline{93.26} & \underline{93.16} & 87.56 & 77.31 & \underline{91.2} & 78.5 & \underline{86.83} & \underline{95.17}  \\
     & *Segmenter~\cite{segmenter} & 90.39 & 91.17 & 83.96 & 65.43 & 87.8 & 68.17 & 81.15 & 93.22  \\
            \cmidrule{2-10}
     & \textbf{*\ours{}-r8} & \underline{\textbf{95.15}} & \underline{\textbf{94.45}} & \underline{\textbf{89.83}} & \underline{\textbf{86.25}} & \underline{\textbf{91.95}} & \underline{76.86} & \underline{\textbf{89.08}} & \underline{\textbf{95.66}}  \\
    & \textbf{*\ours{}-r16} &  93.68 & 93.95 & 88.73 & 83.86 & 90.86 & 71.36 & 87.07 & 94.99 \\
    & \textbf{*\ours{}-r32} & 92.76 & 93.28 & 87.44 & 79.9 & 89.55 & 66.46 & 84.9 & 94.24 \\
    
    
  
    

%   \midrule
  \midrule
% \cmidrule{1-9}
     \multirow{11}[5]{*}{RELLIS-3D} & PSPNet \cite{zhao2017pyramid} & 69.21 & 80.99 & 8.89 & 53.7 & 60.7 & \underline{94.67} & 61.36 & 86.01 \\
    %  & DeepLabv3+ \cite{deeplabv3+} & 65.76 & 79.84 & 19.72 & 47.52 & 64.88 & 95.92 & 62.27 & 85.84\\
    %  & DANet \cite{fu2019dual} & 72.93 & \underline{85.18} & 13.10 & \underline{60.60} & 70.53 & \underline{95.95} & 66.38 & \underline{89.11}\\
     & OCRNet \cite{yuan2020objectcontextual} & \underline{74.67} & \underline{83.04} & 27.76 & \underline{60.44} & 62.35 & 92.58 & 66.81 & \underline{86.95}\\
    %  & PSANet \cite{2018psanet} & 64.06 & 75.29 & 17.08 & 47.45 & 61.74 & 94.31 & 59.99 & 83.17 \\
     
    %  & BiseNetv2~\cite{bisenetv2} & 65.56 & 73.24 & 39.35 & 48.17 & \underline{71.91} & 93.78 & 65.33 & 83.03    \\
     & CGNet~\cite{cgnet} & 62.84 & 74.17 & 49.57 & 45.41 & 68.88 & 94.53 & 65.9 & 82.7 \\
     & FastSCNN~\cite{fastscnn} & 67.06 & 77.6 & \underline{\textbf{56.49}} & 49.76 & \underline{70.31} & 94.43 & \underline{69.27} & 84.51 \\
    %  & FastFCN~\cite{fastfcn} & 70.51 & 79.15 & \underline{49.72} & 51.37 & 63.9 & 94.82 & 68.24 & 84.1 \\            
    % \cmidrule{2-10}
     & *SETR~\cite{setr} & 65.37 & 78.64 & 40.89 & 52.59 & 63.8 & 91.87 & 65.53 & 83.59 \\
     & *DPT~\cite{dpt} & 5.42 & 76.65 & 47.13 & 54.87 & 62.74 & 85.5 & 55.38 & 81.61 \\
     & *Segformer~\cite{segformer} & 60.28 & 79.78 & 53.35 & 53.78 & 70.15 & 94.37 & 68.62 & 85.37\\
     & *Segmenter~\cite{segmenter} & 51.67 & 78.4 & 19.38 & 42.61 & 66.04 & 92.05 & 58.36 & 82.16\\
            \cmidrule{2-10}
     & \textbf{*\ours{}-r8} & \underline{\textbf{78.5}} & \underline{\textbf{88.25}} & \underline{37.28} & \underline{\textbf{72.34}} & \underline{\textbf{74.75}} & \underline{
\textbf{96.07}} & \underline{\textbf{74.44}} & \underline{\textbf{91.69}}  \\
%  77.94  88.25  37.28       72.34       74.75     	96.07  74.44  91.69
    & \textbf{*\ours{}-r16} &  78.37 & 85.58 & 28.63 & 67.55 & 73.82 & 95.73 & 71.62 & 90.26\\
    & \textbf{*\ours{}-r32} & 76.73 & 86.86 & 23.49 & 71.58 & 71.24 & 94.65 & 70.76 & 90.44 \\
    
 

  \bottomrule[2 pt]
%   \bottomrule
\end{tabular}

\end{adjustbox}
\caption{\textbf{Comparison with state-of-the-art methods on RUGD and RELLIS-3D:} We compare the performance of our method with transformer-based methods (with *) as well as other methods in terms of IoU and aAcc. \ours{} improves the state-of-the-art mIoU by \rt{$13.47\%$}
% $2.25-39.05\%$
on RUGD and \rt{$10.54\%$}
% $5.17-19.06\%$ 
on RELLIS-3D \rt{on average}. Further, we show that our grouping method can improve the accuracy of classes like smooth region, bumpy region, and forbidden regions by large margins, thus improving safe navigation. We bold the best number and underline one best result from our method and one from other methods. The suffix of our method shows different designs of our network. For example, ``r8" means we reduce height and width of the spatial resolution by a factor of 8 at the spatial alignment step.}
\vspace{-6mm}
\label{tab:comparison}
\end{table*}

==> Tables/comparison_back.tex <==
\begin{table*}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\centering
\vspace{7pt}
\setlength{\tabcolsep}{3mm}
\ra{1.05}
\Large
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{} llcccccccc @{}}
  \toprule[2pt]
     &&&&$4$ Groups&&&&\\ 
  \midrule
  {Dataset} & {Methods (IoU)} &  \multicolumn{2}{c}{Navigable Region} &  \multicolumn{2}{c}{Forbidden Region} & {Obstacle} & {Background} & {mIoU} & {aAcc}\\
  
  \midrule

     \multirow{6}[3]{*}{RUGD} & PSPNet \cite{zhao2017pyramid}  & \multicolumn{2}{c}{90.22}& \multicolumn{2}{c}{60.56}  & 88.82 & 79.06 & 79.66 & 93.91\\
     & DeepLabv3+ \cite{deeplabv3+} & \multicolumn{2}{c}{90.47} & \multicolumn{2}{c}{57.64}   & \underline{\textbf{89.35}} & \underline{\textbf{82.33}} & 79.94 & \underline{\textbf{94.27}}\\
     & DANet \cite{fu2019dual}& \multicolumn{2}{c}{90.0} & \multicolumn{2}{c}{66.84}  & 89.19 & 79.33 & 81.56 & 94.18\\
     & OCRNet \cite{yuan2020objectcontextual} & \multicolumn{2}{c}{89.94}  & \multicolumn{2}{c}{66.29} & 88.24 & \underline{79.54} & 81.0 & 93.7\\
     & PSANet \cite{2018psanet} & \multicolumn{2}{c}{\underline{90.48}} & \multicolumn{2}{c}{\underline{68.92}}  & 88.96 & 79.39 & \underline{81.94} & 94.02\\
     & \ours\   (ours) & \multicolumn{2}{c}{\underline{\textbf{91.1}}}  & \multicolumn{2}{c}{\underline{\textbf{71.37}}} & \underline{89.28} & 79.44 & \underline{\textbf{82.8}} & \underline{ 94.25}\\
%   & \ours\ with DW  (ours) & x & x & x & x & x & x & x & x\\
  \midrule
     \multirow{6}[3]{*}{RELLIS-3D} & PSPNet \cite{zhao2017pyramid} & \multicolumn{2}{c}{79.11} & \multicolumn{2}{c}{\underline{46.94}} & 72.18 & 94.11 & 73.09 & 85.13\\
     & DeepLabv3+ \cite{deeplabv3+} & \multicolumn{2}{c}{70.36}& \multicolumn{2}{c}{42.71} & \underline{\textbf{74.57}} & \underline{95.39} & 70.76 & 82.28\\
     & DANet \cite{fu2019dual} & \multicolumn{2}{c}{75.89} & \multicolumn{2}{c}{43.75} & 69.27 & 94.5 & 70.85 & 83.26\\
     & OCRNet \cite{yuan2020objectcontextual} & \multicolumn{2}{c}{\underline{80.18}} & \multicolumn{2}{c}{44.57} & \underline{73.99} & 95.17 & \underline{73.48} & \underline{85.73}\\
     & PSANet \cite{2018psanet} & \multicolumn{2}{c}{77.3} & \multicolumn{2}{c}{46.52} & 72.91 & 94.94 & 72.91 & 84.56\\
    %  & \ours\  (ours) & 72.35 & 84.13 & 28.04 & 62.20 & 67.38 & 95.50 & 68.27 & 88.77 \\
    %  & \ours\ with DW (ours) & 73.63 & 86.72 & 29.08 & 67.33 & 71.49 & 95.52 & 70.63 & 90.23 \\
     & \ours\ (ours) & \multicolumn{2}{c}{\underline{
     \textbf{85.9}}} & \multicolumn{2}{c}{\underline{\textbf{59.67}}} & 69.15 & \underline{\textbf{95.56}} & \underline{\textbf{77.57}} & \underline{\textbf{89.8}}\\





%   \midrule[2pt]
%  &&&&$4$ Groups&&&&\\ 
%   \midrule
%      \multirow{6}[3]{*}{RUGD} & PSPNet \cite{zhao2017pyramid}  & 90.22 & - & - & 60.56 & 88.82 & 79.06 & 79.66 & 93.91\\
%      & DeepLabv3+ \cite{deeplabv3+} & 90.47 & - & -  & 57.64 & \textbf{89.35} & 82.33 & 79.94 & \textbf{94.27}\\
%      & DANet \cite{fu2019dual}& 90.0 & - & - & 66.84 & 89.19 & 79.33 & 81.56 & 94.18\\
%      & OCRNet \cite{yuan2020objectcontextual} & 89.94 & - & - & 66.29 & 88.24 & \textbf{79.54} & 81.0 & 93.7\\
%      & PSANet \cite{2018psanet} & 90.48 & - & - & 68.92 & 88.96 & 79.39 & 81.94 & 94.02\\
%      & \ours\   (ours) & \textbf{91.1} & - & - & \textbf{71.37} & 89.28 & 79.44 & \textbf{82.8} & 94.25\\
% %   & \ours\ with DW  (ours) & x & x & x & x & x & x & x & x\\
%   \midrule
%      \multirow{6}[3]{*}{RELLIS-3D} & PSPNet \cite{zhao2017pyramid} & 79.11 & - & - & 46.94 & 72.18 & 94.11 & 73.09 & 85.13\\
%      & DeepLabv3+ \cite{deeplabv3+} & 70.36 & - & - & 42.71 & \textbf{74.57} & 95.39 & 70.76 & 82.28\\
%      & DANet \cite{fu2019dual} & 75.89 & - & - & 43.75 & 69.27 & 94.5 & 70.85 & 83.26\\
%      & OCRNet \cite{yuan2020objectcontextual} & 80.18 & - & - & 44.57 & 73.99 & 95.17 & 73.48 & 85.73\\
%      & PSANet \cite{2018psanet} & 77.3 & - & - & 46.52 & 72.91 & 94.94 & 72.91 & 84.56\\
%     %  & \ours\  (ours) & 72.35 & 84.13 & 28.04 & 62.20 & 67.38 & 95.50 & 68.27 & 88.77 \\
%     %  & \ours\ with DW (ours) & 73.63 & 86.72 & 29.08 & 67.33 & 71.49 & 95.52 & 70.63 & 90.23 \\
%      & \ours\ (ours) & \textbf{85.9} & - & - & \textbf{59.67} & 69.15 & \textbf{95.56} & \textbf{77.57} & \textbf{89.8}\\





  \bottomrule[2 pt]
\end{tabular}

\end{adjustbox}
\caption{\textbf{Some comparisons with state-of-the-art methods on RUGD and RELLIS-3D with 4 terrain classes:} We highlight the results and improvements using 4 terrain classes. We underline the best and second-best results and bold the best number.}
% \vspace{-5mm}
\label{tab:comparison_back}
\end{table*}

==> Tables/dynamic_weight.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
  \toprule
   Backbone & Grouping & Dynamic weighting    & mIoU & mAcc & aAcc \\
  \midrule
  PSANet & & & 46.65 & 53.2 & 89.04\\ 
  PSANet &  & \checkmark  & 50.35 & 66.74 & 87.48\\ 
  \midrule
   PSANet & \checkmark & & 60.32 & 64.32 & 91.52\\ 
  PSANet &  \checkmark & \checkmark  & 79.26 & 89.43 & 93.47 \\ 
 \bottomrule
\end{tabular}
}
\caption{Dynamic weighting effect}

\label{tab:dynamic_weight}

% \vspace{-11mm}
\end{table}

==> Tables/error_rate.tex <==

% \begin{table*}
% \centering
% \caption{\textbf{Error rate analysis with grouping:}   }
% \resizebox{\linewidth}{!}{%
% \makebox[\textwidth][c]{
% \begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
% \toprule[1.1pt]
%  Methods   & &
% \multicolumn{3}{c|}{Smooth Navigable Region}
% &
% \multicolumn{3}{c|}{Rough Navigable Region}
% &
% \multicolumn{3}{c|}{Bumpy Region}      
% &
% \multicolumn{3}{c|}{Forbidden Region}
% &
% \multicolumn{3}{c|}{Obstacle}
% &
% \multicolumn{3}{c}{Background}   
% \\
% \midrule
% x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\

% %                     &
% % \multicolumn{2}{c}{CS-LSTM }         &
% % \multicolumn{2}{c}{TraPHic  }         &
% % \multicolumn{2}{c}{Social-GAN  }         &
% % \multicolumn{2}{c}{GRIP  }         &
% % \multicolumn{2}{c}{S1 Only }  &
% % \multicolumn{2}{c}{S1 + S2 \Tstrut }            \\


% % \midrule
% % &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE \\
% % \midrule
% % \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}z
% % Lyft (5 sec.)           &   4.423  &  8.640  & 5.031  &  9.882   &  7.860  &  14.340  & -  &  - & 5.77  &  11.20  &  \textbf{2.65} &  \textbf{2.99}\\ 
% % Argoverse (5 sec.)      &    1.050  &  3.085  & 1.039  &  3.079   &  3.610   &  5.390  & -  &- &  2.40 &  3.09  &  \textbf{0.99} &  \textbf{1.87} \\ 
% % Apolloscape (3 sec.)    &    2.144  &  11.699  & 1.283  &  11.674  & 3.980  & 6.750  & 1.25 &  2.34  & 2.14  & 9.19  &  \textbf{1.12} &  \textbf{2.05}\\ 
% % NGSIM (5 sec.)  &   7.250&10.050  & 5.630&9.910  & 5.650&10.290  & 1.61  &  3.16  &  1.31  &  2.98  &\textbf{0.40}  & \textbf{1.08}\\ 


% \bottomrule[1.1pt]
% \end{tabular}
% }
% }
% \label{tab: accuracy}
% % \vspace{-15pt}
% \end{table*}


% \begin{table*}[t]
% % \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
% \centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{@{}lcccccccccccccc@{}}
%   \toprule[2pt]
%   \multirow{2}[3]{*}{Groups (Accuracy)} &&
%   \multicolumn{3}{c}{PSPNet \cite{zhao2017pyramid}}&& 
%   \multicolumn{3}{c}{DeepLabv3+ \cite{deeplabv3+}}&&  
%   \multicolumn{3}{c}{OCRNet \cite{yuan2020objectcontextual}}\\
%   \cmidrule(l{3mm}r{3mm}){3-5} 
%   \cmidrule(l{3mm}r{3mm}){7-9} 
%   \cmidrule(l{3mm}r{3mm}){11-13}
%   && {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%) &&  {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%) &&  {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%)\\
% %   \midrule
% %   \midrule
% \midrule[2pt]
%  &&&&&&$6$ Groups&&&&&&\\ 
%   \midrule
%   Smooth Navigable Region && 
%     8.36 & 50.95 & \textbf{42.59} && 
%     4.88 & 5.94 & 1.06 && 
%     58.94 & 70.65 & 11.71 \\ 
%   Rough Navigable Region && 
%     95.4 & 95.05 & $-$0.35 && 
%     92.21 & 95.98 & 3.77 && 
%     93.32 & 96.1 & 2.78 \\ 
%   Bumpy Region && 
%     19.81 & 81.46 & \textbf{61.65} && 
%     15.67 & 74.67 & \textbf{59} && 
%     51.65 & 91.56 & \textbf{39.91} \\ 
%   Forbidden Region && 
%     46.35 & 65.47 & \textbf{19.12} && 
%     68.7 & 71.74 & 3.04 && 
%     51.12 & 71.85 & \textbf{20.73} \\ 
%   Obstacle && 
%     93.84 & 94.03 & 0.19  && 
%     95.61 & 92.16 & $-$3.45 && 
%     93.08 & 93.57 & 0.49 \\ 
%   Background  && 
%     84.8 & 85.73 & 0.93 && 
%     85.62 & 86.93 & 1.31 && 
%     82.49 & 86.11 & 3.62 \\ 
%   \midrule
% mean IoU  && 
% 50.16 & 67.06 & \textbf{16.9} && 
% 47.14 & 55.88 & 8.74 && 
% 64.05 & 76.5 & \textbf{12.45} \\ 
% mean accuracy (per class)  && 
% 58.09 & 78.78 & \textbf{20.69} && 
% 60.45 & 71.24 & \textbf{10.79} && 
% 71.77 & 84.97 & \textbf{13.2} \\ 
%   All pixels accuracy && 
%     91.8 & 92.85 & 1.05 && 
%     91.48 & 91.51 & 0.03 && 
%     91.47 & 93.46 & 1.99 \\ 
%   \midrule[2pt]
% %   \midrule
%  &&&&&&$4$ Groups&&&&&&\\ 
%   \midrule
%   Navigable Region && 
%     95.36 & 96.96 & x && 
%     89.57 & 96.77 & x && 
%     92.47 & 96.28 & x  \\ 
%   Forbidden Region && 
%     46.35 & 75.18 & x && 
%     68.7 & 76.78 & x && 
%     67.8 & 73.93 & x  \\ 
%   Obstacle && 
%     93.84 & 93 & x && 
%     95.61 & 93.15 & x && 
%     95.83 & 93.52 & x  \\ 
%   Background  && 
%     84.8 & 86.2 & x && 
%     85.62 & 89.26 & x && 
%     80.05 & 85.63 & x  \\ 
%   \midrule
% mean IoU  && 
%     70.03 & 82.44 & x && 
%     66.41 & 83.1 & x && 
%     77.95 & 81.82 & x  \\ 
% mean accuracy (per class)  && 
%     80.09 & 87.84 & x && 
%     84.88 & 88.99 & x && 
%     84.04 & 87.34 & x  \\ 
%   All pixels accuracy && 
%     93.66 & 94.01 & x && 
%     92.31 & 94.27 & x && 
%     93.11 & 93.95 & x  \\ 

%   \bottomrule[2pt]
% \end{tabular}

% \end{adjustbox}
% \caption{\textbf{Effect of grouping on the RUGD test set:} The first column under each method shows the results on the 24-class setting, the second column shows results on the 6-column setting and the third column shows the improvement that the grouping scheme imparts to the network. We show how training by grouping can improve performance of segmentation models thus proving that grouping is indeed beneficial. }
% % \vspace{-6mm}
% \label{tab:error}
% \end{table*}


\begin{table}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\centering
\vspace{10pt}
\setlength{\tabcolsep}{3mm}
\ra{1.05}
\Large
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{@{}lccccccc@{}}
  \toprule[2pt]
  Groups (Accuracy) & OCRNet \cite{yuan2020objectcontextual} & OCR-G && GANav (ours) \\
  %\multirow{2}[3]{*}{Groups (Accuracy)} &
  %\multicolumn{2}{c}{OCRNet \cite{yuan2020objectcontextual}}&& %\multicolumn{2}{c}{\ours\  (ours) }\\
  %\cmidrule(l{3mm}r{3mm}){2-3} 
  %\cmidrule(l{2mm}r{0.01mm}){5-5} 
  % & {w/o. Grouping} & {w. Grouping} & & {w. Grouping} \\
%   \midrule
%   \midrule
%   \midrule

\midrule[2pt]
 &$6$ Groups&&\\ 
%   \midrule
%   Smooth Navigable Region && 
%     8.36 & 50.95 && 
%     58.94 & 70.65 \\ 
%   Rough Navigable Region && 
%     95.4 & 95.05  && 
%     93.32 & 96.1  \\ 
%   Bumpy Region && 
%     19.81 & 81.46 && 
%     51.65 & 91.56  \\ 
%   Forbidden Region && 
%     46.35 & 65.47  && 
%     51.12 & 71.85 \\ 
%   Obstacle && 
%     93.84 & 94.03   && 
%     93.08 & 93.57 \\ 
%   Background  && 
%     84.8 & 85.73 && 
%     82.49 & 86.11 \\ 
  \midrule
mean IoU  &
64.05 & 76.5  && 
83.24\\ 
mean accuracy (per class)  & 
71.77 & 84.97  && 
 89.84  \\ 
  All pixels accuracy & 
    91.47 & 93.46  && 
94.26  \\ 
\midrule[2pt]
 &$4$ Groups&&\\ 
  \midrule
%   Navigable Region && 
%     95.36 & 96.96 && 
%     92.47 & 96.28 \\ 
%   Forbidden Region && 
%     46.35 & 75.18  && 
%     67.8 & 73.93 \\ 
%   Obstacle && 
%     93.84 & 93  && 
%     95.83 & 93.52   \\ 
%   Background  && 
%     84.8 & 86.2 && 
%     80.05 & 85.63  \\ 
%   \midrule
mean IoU  & 
    77.95 & 81.0  && 
 82.8   \\ 
mean accuracy (per class)  & 
    84.04 & 88.0  && 
 89.14   \\ 
  All pixels accuracy & 
    93.11 & 93.7  && 
 94.25  \\ 

%   \midrule[2pt]

  \bottomrule[2pt]
\end{tabular}

\end{adjustbox}
\caption{\textbf{Effect of grouping on the RUGD test set:} The first column shows the results of the current SOTA method OCRNet \cite{yuan2020objectcontextual} on the 24-class setting, and the second column shows the results of OCRNet \cite{yuan2020objectcontextual} on our newly proposed taxonomy. We show how training by grouping can improve the performance of segmentation models, thus proving that grouping is indeed beneficial. In the third column, we show that our architecture results in improved performance over the SOTA.}
% \caption{\textbf{Effect of grouping on the RUGD test set:} The first column under each method shows the results on the 24-class setting and the second column shows results on the 6-class setting. We show how training by grouping can improve performance of segmentation models thus proving that grouping is indeed beneficial. \divya{Change} }
\vspace{-7mm}
\label{tab:error}
\end{table}

==> Tables/error_rate2.tex <==

% \begin{table*}
% \centering
% \caption{\textbf{Error rate analysis with grouping:}   }
% \resizebox{\linewidth}{!}{%
% \makebox[\textwidth][c]{
% \begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
% \toprule[1.1pt]
%  Methods   & &
% \multicolumn{3}{c|}{Smooth Navigable Region}
% &
% \multicolumn{3}{c|}{Rough Navigable Region}
% &
% \multicolumn{3}{c|}{Bumpy Region}      
% &
% \multicolumn{3}{c|}{Forbidden Region}
% &
% \multicolumn{3}{c|}{Obstacle}
% &
% \multicolumn{3}{c}{Background}   
% \\
% \midrule
% x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\

% %                     &
% % \multicolumn{2}{c}{CS-LSTM }         &
% % \multicolumn{2}{c}{TraPHic  }         &
% % \multicolumn{2}{c}{Social-GAN  }         &
% % \multicolumn{2}{c}{GRIP  }         &
% % \multicolumn{2}{c}{S1 Only }  &
% % \multicolumn{2}{c}{S1 + S2 \Tstrut }            \\


% % \midrule
% % &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE \\
% % \midrule
% % \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}z
% % Lyft (5 sec.)           &   4.423  &  8.640  & 5.031  &  9.882   &  7.860  &  14.340  & -  &  - & 5.77  &  11.20  &  \textbf{2.65} &  \textbf{2.99}\\ 
% % Argoverse (5 sec.)      &    1.050  &  3.085  & 1.039  &  3.079   &  3.610   &  5.390  & -  &- &  2.40 &  3.09  &  \textbf{0.99} &  \textbf{1.87} \\ 
% % Apolloscape (3 sec.)    &    2.144  &  11.699  & 1.283  &  11.674  & 3.980  & 6.750  & 1.25 &  2.34  & 2.14  & 9.19  &  \textbf{1.12} &  \textbf{2.05}\\ 
% % NGSIM (5 sec.)  &   7.250&10.050  & 5.630&9.910  & 5.650&10.290  & 1.61  &  3.16  &  1.31  &  2.98  &\textbf{0.40}  & \textbf{1.08}\\ 


% \bottomrule[1.1pt]
% \end{tabular}
% }
% }
% \label{tab: accuracy}
% % \vspace{-15pt}
% \end{table*}


% \begin{table*}[t]
% % \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
% \centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{@{}lcccccccccccccc@{}}
%   \toprule[2pt]
%   \multirow{2}[3]{*}{Groups (Accuracy)} &&
%   \multicolumn{3}{c}{PSPNet \cite{zhao2017pyramid}}&& 
%   \multicolumn{3}{c}{DeepLabv3+ \cite{deeplabv3+}}&&  
%   \multicolumn{3}{c}{OCRNet \cite{yuan2020objectcontextual}}\\
%   \cmidrule(l{3mm}r{3mm}){3-5} 
%   \cmidrule(l{3mm}r{3mm}){7-9} 
%   \cmidrule(l{3mm}r{3mm}){11-13}
%   && {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%) &&  {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%) &&  {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%)\\
% %   \midrule
% %   \midrule
% \midrule[2pt]
%  &&&&&&$6$ Groups&&&&&&\\ 
%   \midrule
%   Smooth Navigable Region && 
%     8.36 & 50.95 & \textbf{42.59} && 
%     4.88 & 5.94 & 1.06 && 
%     58.94 & 70.65 & 11.71 \\ 
%   Rough Navigable Region && 
%     95.4 & 95.05 & $-$0.35 && 
%     92.21 & 95.98 & 3.77 && 
%     93.32 & 96.1 & 2.78 \\ 
%   Bumpy Region && 
%     19.81 & 81.46 & \textbf{61.65} && 
%     15.67 & 74.67 & \textbf{59} && 
%     51.65 & 91.56 & \textbf{39.91} \\ 
%   Forbidden Region && 
%     46.35 & 65.47 & \textbf{19.12} && 
%     68.7 & 71.74 & 3.04 && 
%     51.12 & 71.85 & \textbf{20.73} \\ 
%   Obstacle && 
%     93.84 & 94.03 & 0.19  && 
%     95.61 & 92.16 & $-$3.45 && 
%     93.08 & 93.57 & 0.49 \\ 
%   Background  && 
%     84.8 & 85.73 & 0.93 && 
%     85.62 & 86.93 & 1.31 && 
%     82.49 & 86.11 & 3.62 \\ 
%   \midrule
% mean IoU  && 
% 50.16 & 67.06 & \textbf{16.9} && 
% 47.14 & 55.88 & 8.74 && 
% 64.05 & 76.5 & \textbf{12.45} \\ 
% mean accuracy (per class)  && 
% 58.09 & 78.78 & \textbf{20.69} && 
% 60.45 & 71.24 & \textbf{10.79} && 
% 71.77 & 84.97 & \textbf{13.2} \\ 
%   All pixels accuracy && 
%     91.8 & 92.85 & 1.05 && 
%     91.48 & 91.51 & 0.03 && 
%     91.47 & 93.46 & 1.99 \\ 
%   \midrule[2pt]
% %   \midrule
%  &&&&&&$4$ Groups&&&&&&\\ 
%   \midrule
%   Navigable Region && 
%     95.36 & 96.96 & x && 
%     89.57 & 96.77 & x && 
%     92.47 & 96.28 & x  \\ 
%   Forbidden Region && 
%     46.35 & 75.18 & x && 
%     68.7 & 76.78 & x && 
%     67.8 & 73.93 & x  \\ 
%   Obstacle && 
%     93.84 & 93 & x && 
%     95.61 & 93.15 & x && 
%     95.83 & 93.52 & x  \\ 
%   Background  && 
%     84.8 & 86.2 & x && 
%     85.62 & 89.26 & x && 
%     80.05 & 85.63 & x  \\ 
%   \midrule
% mean IoU  && 
%     70.03 & 82.44 & x && 
%     66.41 & 83.1 & x && 
%     77.95 & 81.82 & x  \\ 
% mean accuracy (per class)  && 
%     80.09 & 87.84 & x && 
%     84.88 & 88.99 & x && 
%     84.04 & 87.34 & x  \\ 
%   All pixels accuracy && 
%     93.66 & 94.01 & x && 
%     92.31 & 94.27 & x && 
%     93.11 & 93.95 & x  \\ 

%   \bottomrule[2pt]
% \end{tabular}

% \end{adjustbox}
% \caption{\textbf{Effect of grouping on the RUGD test set:} The first column under each method shows the results on the 24-class setting, the second column shows results on the 6-column setting and the third column shows the improvement that the grouping scheme imparts to the network. We show how training by grouping can improve performance of segmentation models thus proving that grouping is indeed beneficial. }
% % \vspace{-6mm}
% \label{tab:error}
% \end{table*}


\begin{table*}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\centering
\setlength{\tabcolsep}{3mm}
\ra{1.05}
\Large
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}lcccccccccccccc@{}}
  \toprule[2pt]
  \multirow{2}[3]{*}{Groups (Accuracy)} &&
  \multicolumn{3}{c}{PSPNet \cite{zhao2017pyramid}}&& 
  \multicolumn{3}{c}{DeepLabv3+ \cite{deeplabv3+}}&&  
  \multicolumn{3}{c}{OCRNet \cite{yuan2020objectcontextual}}\\
  \cmidrule(l{3mm}r{3mm}){3-5} 
  \cmidrule(l{3mm}r{3mm}){7-9} 
  \cmidrule(l{3mm}r{3mm}){11-13}
  && {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%) &&  {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%) &&  {w/o. Grouping} & {w. Grouping} & $\uparrow$(\%)\\
%   \midrule
%   \midrule
\midrule[2pt]
 &&&&&&$6$ Groups&&&&&&\\ 
  \midrule
  Smooth Navigable Region && 
    8.36 & 50.95 & \textbf{42.59} && 
    4.88 & 5.94 & 1.06 && 
    58.94 & 70.65 & \textbf{11.71} \\ 
  Rough Navigable Region && 
    95.4 & 95.05 & $-$0.35 && 
    92.21 & 95.98 & 3.77 && 
    93.32 & 96.1 & 2.78 \\ 
  Bumpy Region && 
    19.81 & 81.46 & \textbf{61.65} && 
    15.67 & 74.67 & \textbf{59} && 
    51.65 & 91.56 & \textbf{39.91} \\ 
  Forbidden Region && 
    46.35 & 65.47 & \textbf{19.12} && 
    68.7 & 71.74 & 3.04 && 
    51.12 & 71.85 & \textbf{20.73} \\ 
  Obstacle && 
    93.84 & 94.03 & 0.19  && 
    95.61 & 92.16 & $-$3.45 && 
    93.08 & 93.57 & 0.49 \\ 
  Background  && 
    84.8 & 85.73 & 0.93 && 
    85.62 & 86.93 & 1.31 && 
    82.49 & 86.11 & 3.62 \\ 
  \midrule
mean IoU  && 
50.16 & 67.06 & \textbf{16.9} && 
47.14 & 55.88 & 8.74 && 
64.05 & 76.5 & \textbf{12.45} \\ 
mean accuracy (per class)  && 
58.09 & 78.78 & \textbf{20.69} && 
60.45 & 71.24 & \textbf{10.79} && 
71.77 & 84.97 & \textbf{13.2} \\ 
  All pixels accuracy && 
    91.8 & 92.85 & 1.05 && 
    91.48 & 91.51 & 0.03 && 
    91.47 & 93.46 & 1.99 \\ 
  \midrule[2pt]
%   \midrule
 &&&&&&$4$ Groups&&&&&&\\ 
  \midrule
  Navigable Region && 
    95.36 & 95.17 & $-$0.19 && 
    89.57 & 96.03 & 6.46 && 
    92.47 & 96.88 & 4.41  \\ 
  Forbidden Region && 
    46.35 & 76.35 & \textbf{30} && 
    68.7 & 79.42 & \textbf{10.72} && 
    67.8 & 75.71 & 7.91  \\ 
  Obstacle && 
    93.84 & 94.49 & 0.65 && 
    95.61 & 93.72 & $-$1.89 && 
    95.83 & 92.32 & $-$3.51  \\ 
  Background  && 
    84.8 & 84.65 & $-$0.15 && 
    85.62 & 89.38 & 3.76 && 
    80.05 & 87.09 & 7.04 \\ 
  \midrule
mean IoU  && 
    70.03 & 79.66 & 9.63 && 
    66.41 & 79.94 & \textbf{13.53} && 
    77.95 & 81.0 & 3.05 \\ 
mean accuracy (per class)  && 
    80.09 & 87.66 & 7.57 && 
    84.88 & 89.64 & 4.76 && 
    84.04 & 88.0 & 3.96 \\ 
  All pixels accuracy && 
    93.66 & 93.91 & 0.25 && 
    92.31 & 94.27 & 1.96 && 
    93.11 & 93.7 & 0.59  \\ 

  \bottomrule[2pt]
\end{tabular}

\end{adjustbox}
\caption{\textbf{Effect of grouping on the RUGD test set:} The first column under each method shows the results on the 24-class setting, the second column shows results on the 6-class setting, and the third column shows the improvement that the grouping scheme imparts to the network. }
% \vspace{2mm}
\label{tab:error2}
\end{table*}

==> Tables/realworld_sup.tex <==


% \begin{table}[t]
% % \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
% \centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{@{}cccc@{}}
%   \toprule[2pt]
%   Measuerment for Navigation & OCRNet \cite{yuan2020objectcontextual} & PSPNet \cite{zhao2017pyramid} & GANav (ours) \\
%   \midrule

% Success Rate  &
% 1 / 6 & 0 / 6  &
% 5 / 6 \\ 
% %   \midrule
% Averaged Progress towards Goal  & 
% 14.59\% & 15.92\% & 85.99\%  \\ 


%   \midrule

% 5071 / 12690
% 3914 / 12690
% 112 / 12690



%   \midrule[2pt]

% %   \bottomrule[2pt]
% \end{tabular}

% \end{adjustbox}
% \caption{\textbf{Detailed navigation results}}
% \vspace{-3mm}
% \label{tab:breakdown}
% \end{table}


\begin{table}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\centering
\setlength{\tabcolsep}{3mm}
\ra{1.05}
\Large
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{@{} llccc @{}}
  \toprule[2pt]
  {Scenario} &
  {Metrics} & {PSPNet \cite{zhao2017pyramid}} & {OCRNet \cite{yuan2020objectcontextual}} & {\ours\   (ours)} \\
  
  \midrule


     \multirow{3}[1]{*}{Route 1} & Reach Goal? &   &  & \checkmark \\
     & Time-until-Failure (s) & 2  & 4 & - \\
     & Progress towards Goal (\%) & 4.44 & 8.89 & 100 \\

  \midrule


     \multirow{3}[1]{*}{Route 2} & Reach Goal? &   &  & \checkmark \\
     & Time-until-Failure (s) & 0  & 6 & - \\
     & Progress towards Goal (\%) & 0 & 15 & 100 \\
     
     
  \midrule


     \multirow{3}[1]{*}{Route 3} & Reach Goal? &   &  & \checkmark \\
     & Time-until-Failure (s) & 0  & 4 & - \\
     & Progress towards Goal (\%) & 0 & 5.19 & 100 \\

  \midrule


     \multirow{3}[1]{*}{Route 4} & Reach Goal? &   &  & \checkmark \\
     & Time-until-Failure (s) & 45  & 40 & - \\
     & Progress towards Goal (\%) & 47.87 & 42.55 & 100 \\

  \midrule


     \multirow{3}[1]{*}{Route 5} & Reach Goal? &   & \checkmark & \checkmark \\
     & Time-until-Failure (s) & 15  & - & - \\
     & Progress towards Goal (\%) & 27.27 & 100 & 100 \\
     
     
  \midrule


     \multirow{3}[1]{*}{Route 6} & Reach Goal? &   &  &  \\
     & Time-until-Failure (s) & 7  & 7 & 7 \\
     & Progress towards Goal (\%) & 15.91 & 15.91 & 15.91 \\
% psp 2/45, 0/40, 0/77, 45/94, 15/55, 7/44
% ocr 4/45, 6/40, 4/77, 40/94, 55/55,  7/44
% ganav 100/100,  100/100, 100/100, 100/100, 100/100, 7/44
% 4.44, 0, 0, 47.87, 27.27, 15.91 = 15.92
% 8.89, 15, 5.19, 42.55, 100, 15.91 = 31.26
% 100, 100, 100, 100, 100, 15.91 = 85.99

  \bottomrule[2 pt]
\end{tabular}

\end{adjustbox}
\caption{\textbf{Detailed Navigation Results with Jackal:} We show our different testing scenarios and navigation results of each trial. }
\vspace{-3mm}
\label{tab:breakdown}
\end{table}

==> Tables/runtime.tex <==

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc}
  \toprule
 \multirow{2}[0]{*}{\textbf{Method}}  & \textbf{Params $\downarrow$} & \multirow{2}[0]{*}{\textbf{GFLOPS $\downarrow$}} & \textbf{Inf Mem $\downarrow$} & \textbf{Run-time $\uparrow$} \\
 & \textbf{(M)} & & \textbf{(MiB)} &\textbf{(img/s)}\\
%   \textbf{Method}  & \textbf{Params (M) $\downarrow$} & \textbf{GFLOPS $\downarrow$} & \textbf{Inf Mem (MiB)} $\downarrow$ & \textbf{Run-time (img / s)} $\uparrow$ \\
  \midrule
  
PSPNet \cite{zhao2017pyramid}  & 48.97 & 258.9 & 1635 & 21.97 \\
% DeepLabv3+ \cite{deeplabv3+}  & 43.58 & 256.08 & 1443 & 43.48 \\
% DANet \cite{fu2019dual}  & 49.82 & 288.81 & 1425 & 29.97 \\
OCRNet \cite{yuan2020objectcontextual} & 36.51 & 221.47 & 1407 & 20.76\\
% PSANet \cite{2018psanet}  & 59.13 & 289.52 & 1629 & 28.26 \\
% BiseNetv2~\cite{bisenetv2}  & 14.78 & 17.88 & 1137 & 90.33\\
CGNet~\cite{cgnet}  & \underline{0.493} & 5.05 & 1087 & 62.35\\
FastSCNN~\cite{fastscnn}  & 1.45 & \underline{1.35} & \underline{1081} & \underline{110.63}\\
% FastFCN~\cite{fastfcn}  & 68.7 & 189.61 & 1707 & 47.83\\
\midrule
*SETR~\cite{setr}  & 309.17 & 312.21 & 2295 & 22.96\\
*DPT~\cite{dpt}  & 109.67 & 255.49 & 1633 & 37.03 \\
*Segformer~\cite{segformer}  & \underline{3.72} & 9.29 & 1143 & \underline{73.49}\\
*Segmenter~\cite{segmenter}  & 6.69 & \underline{6.57} & \underline{1109} & 52.72\\
\midrule
\textbf{*\ours{}-r8}  & 6.94 & 18.69 & 1415 & 65.53\\
\textbf{*\ours{}-r16} & 6.57 & 7.7 & \underline{1121} & 76.20\\
\textbf{*\ours{}-r32}  & \underline{6.21} & \underline{4.54} & 1131 & \underline{76.74}\\
  
  \bottomrule
\end{tabular}
}
\caption{\textbf{Model Complexity:} We show the model parameter size, GLOPS, GPU memory cost during inference, and run-time. For each measurement, we underline one best number among CNN-based methods, one among transformer-based methods, and one among variations of \ours{}.
}

\label{tab:runtime}

\vspace{-6mm}
\end{table}



% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{cccccc}
%   \toprule
%  \textbf{Method} & \textbf{mIoU (\%) $\uparrow$}   & \textbf{Params (M) $\downarrow$} & \textbf{GFLOPS $\downarrow$} & \textbf{Inf Mem (MiB)} $\downarrow$ & \textbf{Run-time (img / s)} $\uparrow$ \\
%   \midrule
  
% PSPNet \cite{zhao2017pyramid} & 67.06 & 48.97 & 258.9 & 1635 & 21.97 \\
% DeepLabv3+ \cite{deeplabv3+} & 55.88 & 43.58 & 256.08 & 1443 & 43.48 \\
% DANet \cite{fu2019dual} & 44.14 & 49.82 & 288.81 & 1425 & 29.97 \\
% OCRNet \cite{yuan2020objectcontextual} & 76.50 & 36.51 & 221.47 & 1407 & 20.76\\
% PSANet \cite{2018psanet} & 55.47 & 59.13 & 289.52 & 1629 & 28.26 \\
% BiseNetv2~\cite{bisenetv2} & 75.1 & 14.78 & 17.88 & 1137 & 90.33\\
% CGNet~\cite{cgnet} & 76.22 & 0.493 & 5.05 & 1087 & 62.35\\
% FastSCNN~\cite{fastscnn} & 85.11 & 1.45 & 1.35 & 1081 & 110.63\\
% FastFCN~\cite{fastfcn} & 75.51 & 68.7 & 189.61 & 1707 & 47.83\\
% \midrule
% *SETR~\cite{setr} & 82.86 & 309.17 & 312.21 & 2295 & 22.96\\
% *DPT~\cite{dpt} & 49.13 & 109.67 & 255.49 & 1633 & 37.03 \\
% *Segformer~\cite{segformer} & 86.83 & 3.72 & 9.29 & 1143 & 73.49\\
% *Segmenter~\cite{segmenter} & 81.15 & 6.69 & 6.57 & 1109 & 52.72\\
% \midrule
% \textbf{*\ours{}-r8} & 88.49 & 6.94 & 18.69 & 1415 & 65.53\\
% \textbf{*\ours{}-r16} & 87.07 & 6.57 & 7.7 & 1121 & 76.20\\
% \textbf{*\ours{}-r32} & 84.9 & 6.21 & 4.54 & 1131 & 76.74\\
  

%   \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Performance vs. Efficiency:} We show the mIoU performance on RUGD dataset, model parameter size, GLOPS, GPU memory cost during inference, and run-time. 
% }

% \label{tab:runtime}

% \vspace{-2mm}
% \end{table}




==> legacy/root.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %2345678901234567890123456789012345678901234567890123456789012345678901234567890
% %        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}  % Comment this line out if you need a4paper

% %\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper

% \IEEEoverridecommandlockouts                              % This command is only needed if 
%                                                           % you want to use the \thanks command

% \overrideIEEEmargins                                      % Needed to meet printer requirements.

% %In case you encounter the following error:
% %Error 1010 The PDF file may be corrupt (unable to open PDF file) OR
% %Error 1000 An error occurred while parsing a contents stream. Unable to analyze the PDF file.
% %This is a known problem with pdfLaTeX conversion filter. The file cannot be opened with acrobat reader
% %Please use one of the alternatives below to circumvent this error by uncommenting one or the other
% %\pdfobjcompresslevel=0
% %\pdfminorversion=4

% % See the \addtolength command later in the file to balance the column lengths
% % on the last page of the document

% % The following packages can be found on http:\\www.ctan.org
% %\usepackage{graphics} % for pdf, bitmapped graphics files
% %\usepackage{epsfig} % for postscript graphics files
% %\usepackage{mathptmx} % assumes new font selection scheme installed
% %\usepackage{times} % assumes new font selection scheme installed
% %\usepackage{amsmath} % assumes amsmath package installed
% %\usepackage{amssymb}  % assumes amsmath package installed

% \title{\LARGE \bf
% Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
% }


% \author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
% \thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
%         University of Twente, 7500 AE Enschede, The Netherlands
%         {\tt\small albert.author@papercept.net}}%
% \thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
%         Dayton, OH 45435, USA
%         {\tt\small b.d.researcher@ieee.org}}%
% }


% \begin{document}



% \maketitle
% \thispagestyle{empty}
% \pagestyle{empty}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract}

% This electronic document is a ÒliveÓ template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.

% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{INTRODUCTION}

% This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

% \section{PROCEDURE FOR PAPER SUBMISSION}

% \subsection{Selecting a Template (Heading 2)}

% First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
% It may be used for A4 paper size if the paper size setting is suitably modified.

% \subsection{Maintaining the Integrity of the Specifications}

% The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

% \section{MATH}

% Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

% Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

% \subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

% \subsection{Units}

% \begin{itemize}

% \item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
% \item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
% \item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
% \item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

% \end{itemize}


% \subsection{Equations}

% The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

% $$
% \alpha + \beta = \chi \eqno{(1)}
% $$

% Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

% \subsection{Some Common Mistakes}
% \begin{itemize}


% \item The word ÒdataÓ is plural, not singular.
% \item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
% \item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
% \item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
% \item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
% \item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
% \item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
% \item Do not confuse ÒimplyÓ and ÒinferÓ.
% \item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
% \item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
% \item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

% \end{itemize}


% \section{USING THE TEMPLATE}

% Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

% It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

% \subsection{Headings, etc}

% Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

% \subsection{Figures and Tables}

% Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

% \begin{table}[h]
% \caption{An Example of a Table}
% \label{table_example}
% \begin{center}
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


%   \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       %\includegraphics[scale=1.0]{figurefile}
%       \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%   \end{figure}
   

% Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó

% \section{CONCLUSIONS}

% A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{APPENDIX}

% Appendixes should appear before the acknowledgment.

% \section*{ACKNOWLEDGMENT}

% The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



% \begin{thebibliography}{99}

% \bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
% \bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
% \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% \bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
% \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
% \bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
% \bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
% \bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
% \bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
% \bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
% \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 






% \end{thebibliography}




% \end{document}


==> sections/experiments.tex <==
\section{Results and Analysis}
\label{exp}



\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{fig/dataset2.png}
    % \vspace{-3mm}
    \caption{\textbf{Qualitative Results:} Each row highlights the original image, the ground truth (GT) label, the predictions of two SOTA methods, and the prediction of our method. We observe that our method can detect different navigable regions and is robust with respect to objects with similar colors.}
    % \vspace{-13pt}
    \vspace{-6mm}
    \label{fig:visualisations}
\end{figure}







\subsection{Implementation Details}

We use two off-road terrain datasets, RUGD~\cite{RUGD2019IROS} and RELLIS-3D~\cite{rellis}, as benchmarks for all experiments and comparisons. Optimization is done using a stochastic gradient descent optimizer with a learning rate of 0.01 and a decay of 0.0005. We adopt the polynomial learning rate policy with a power of 0.9. We augment the data with horizontal random flip and random crop. In the ablations and comparisons, for fairness, we benchmark all our models at 240K iterations. For the RUGD dataset, we use a batch size of 8 and a crop size of $300\times375$ (the resolution of the original image is $688\times550$). On the other hand, for the RELLIS-3D dataset, due to the high resolution of the image, we train models with a batch size of 2 and a crop size $375\times600$ (the resolution of the original image is $1920\times1600$). Our implementation is based on MMSeg~\cite{mmseg2020} and will be released.


\begin{figure}[t]
    \vspace{-6mm}
    \centering
    \includegraphics[width = 1.05\columnwidth]{fig/runtime.png}
    \vspace{-7mm}
    \caption{\textbf{Performance vs. Inference Time on RELLIS-3D:} The run-times are calculated based on the average time of 200 images.}
    \label{fig:runtime}
    \vspace{-5mm}
\end{figure}

% \input{Tables/runtime}


\input{Tables/comparison}


We benchmark our models on the standard segmentation metrics: Intersection over Union (IoU), mean IoU (mIoU), mean pixel accuracy (mAcc), and average pixel accuracy (aAcc). 
% For an image $I$, let $P(x, y)$ be the predicted label at pixel location $(x, y)$, $G(x, y)$ be the ground truth label at $(x, y)$, $\mathbbm{1}(X)$ be the indicator function, and $B$ be a set of the class labels:
% \noindent \textbf{Intersection over Union (IoU) for class i:}
% $$IoU_{i} = \frac{\sum_{I}\sum_{x, y} \mathbbm{1}(P(x,y) = i \text{ and } G(x, y) = i) }{\sum_{I}\sum_{x, y} \mathbbm{1}(P(x,y) = i \text{ or } G(x, y) = i) }$$
% \noindent \textbf{Mean IoU (mIoU):} 
% $$mIoU = \frac{\sum_{i} mIoU_i}{\sum_{B} 1}$$
% \noindent \textbf{Mean Pixel Accuracy (mAcc):} 
% $$mAcc = \frac{\sum_{i\in B} (\sum_{I}\sum_{x, y, G(x, y) = i} \mathbbm{1}(P(x,y) = G(x, y)) )}{\sum_{B} 1}$$
% \noindent \textbf{Averaged Pixel Accuracy (aAcc):} 
% $$aAcc = \frac{\sum_{I}\sum_{x, y} \mathbbm{1}(P(x,y) = G(x, y)) }{\sum_{I}\sum_{x, y} 1 }$$
We evaluate our methods with 6 coarse-grain semantic classes: smooth (concrete, asphalt), rough (gravel, grass, dirt), bumpy (small rocks, rock-bed), forbidden (water, bushes), obstacle, and background. Some visualizations for method comparisons are provided in Fig.~\ref{fig:visualisations}. Please refer to the full report~\cite{guan2021ganav} for more qualitative results.






% \input{Tables/error_rate}






% \subsection{Effect of Grouping}
% In this section, we analyze the effect of evaluating models based on our new taxonomy of classes. The empirical results are presented in Table \ref{tab:error}. We measure the effects of grouping with two grouping strategies relevant to navigation:

% \begin{itemize}
%     \item 6 Groups: This grouping includes smooth region, rough region, bumpy region, forbidden region, obstacle, and background, as described in Section~\ref{groupings}. This grouping is useful for smaller robots with less mobility, which prefer smooth regions to rough and bumpy regions for navigation.
%     \item 4 Groups: This grouping combines smooth region, rough region, and bumpy region into navigable region, and the remaining categories remain the same. This grouping is used for large vehicles that can traverse rough and bumpy regions with no issues, but still need to avoid obstacles and forbidden regions like puddles.
% \end{itemize}

% % \paragraph{Experimental setup} We train three benchmark segmentation architectures PSPNet \cite{zhao2017pyramid}, DeepLabv3+ \cite{deeplabv3+}, and OCRNet \cite{yuan2020objectcontextual} under two settings: (i) ungrouped setting (first column under each method in Table~\ref{tab:error}) (ii) grouped setting (second column). We evaluate both models on the grouped scenario and show the improvement of setting $(ii)$ over setting $(i)$ in the third column. 

% \paragraph{Experimental setup} We train one previous SOTA method, OCRNet \cite{yuan2020objectcontextual}, and GANav (ours) under two settings: 6 groups and 4 groups. We evaluate ungrouped scenarios with OCRNet and the grouped scenario on both models. Note that our method only works in the grouped scenario, as group-wise attention requires extensive GPU memory with 24 or 20 original classes. 

% \input{QualitativeResults/qualitative}

% \input{Tables/dynamic_weight}
% \paragraph{Analysis} We show that such a grouping strategy improves the performance of current semantic segmentation approaches in off-road terrains by reducing the error rate (or improving accuracy) in long-tail distributed data. We wish to emphasize the motivation behind this through an example. Consider the classes "concrete" and "asphalt", which are highly similar. Under the ungrouped setting, classifying them separately can lead to errors due to homogeneous feature embeddings. However, under the grouped setting, "asphalt" and "concrete" are categorized within the same group, thus providing the network with more flexibility and better margins for learning feature mappings. 
% More error analysis of grouping with other methods can be find in \ref{error_more}.
% More error analysis of grouping with other methods can be find in the Appendix section of the full report~\cite{our_method}.

%sHowever, the effect of grouping can be model dependent. For instance, through our experiments, we found that PSANet had a higher error rate (or lower accuracy) with grouping. Based on the above observations, we hypothesize that the development of an architecture like BoT-OffNav that leverages this grouping can further improve performance. We validate this hypothesis in the following subsection. \rohan{I think we shuold not mention PSAnet. It weakens our point. }



% 10.85
% 7.46
% 8.09

% 2.85
% 4.01
% 5.85




% Although we should still note that the performance drop still existing with GA heads.




\subsection{Results and State-of-the-art Comparisons}
\label{sota_comp}

% Our method works extremely well on the more complicated grouping (6 groups).
% , on which we will analyze the performance. 

In this section, we focus on comparing our method with several methods~\cite{segformer, segmenter, bisenetv2, fastscnn} with an efficient design and similar model size. The results on different coarse-grain classes are presented in Table \ref{tab:comparison}.
Our architecture improves the state-of-the-art mIoU by $2.25-39.05\%$ on RUGD. We can see that our method has the best overall mIoU scores. While \ours{} does not always give the best results for each separate class and the performance is sometimes close to the second best IoU score, our method has very stable performance for each class. \ours{} performs well in terms of detecting different terrains, while other methods only exhibit good performance on one type of terrains.
Similarly, on the RELLIS dataset, \ours\  shows an improvement of $5.17-19.06\%$ in terms of mIoU. 




% Using the smaller number of groups as opposed to training on all $24$ classes enables us to define separate attention heads for each of the groups, which improves the overall performance. 
% Dynamic weighting used in our group-wise attention model results in an improvement of $2.36\%$ on the RELLIS-3D dataset. Dynamic weighting does not lead to an improvement in performance for RUGD, because it is more effective when the dataset has a long-tailed distribution. 

% The ablation studies are presented in Table \ref{tab:ablation}. To show the effect of varying the backbone architecture, we conduct experiments with ResNet-50, ResNet-101, and BottleNeck Transformer. We observe that better backbones lead to improved accuracies. In addition, we show the impact of our class-wise attention loss, and show that it is bestows the transformer bottlneck model with a relative improvement of $11.4\%$ in mIoU.




\input{Tables/ablation3}

\input{Tables/ablation}
\input{Tables/ablation2}


\subsection{Run-time Analysis and Computational Cost}

In Fig.~\ref{fig:runtime}, we highlight the model efficiency of our method while maintaining SOTA performance. We observe that even if we compromise the performance for inference rate in \ours{}-r16 and \ours{}-r32, our method still outperforms other methods in terms of mIoU. 

% Please refer to the full report~\cite{guan2021ganav} for more details.

% In Table~\ref{tab:runtime}, we give more details on model parameter size, GFLOPS, cost during inference, and run-time. While our method doesn't always have the smallest model size and GLOPS, our method has a very low memory requirement. Our method also has the best inference time among listed transformer-based methods and most of the CNN-based methods, given that our method achieves state-of-the-art accuracy, as shown in Section~\ref{sota_comp}.






% \begin{figure}[t]
%     \centering
%     \includegraphics[width = \columnwidth]{fig/realworld_cmp2.png}
%     % \vspace{-3mm}
%     \caption{\textbf{Qualitative Results:} We show the real-world performance of \ours{} and two SOTA methods with pre-trained model on RUGD and RELLIS-3D. The green trajectory is the path of the robot in next 2 seconds based on current velocity. While other methods have some false positive on forbidden region and over-generalize on rough region (in yellow), our method can correctly identify different regions and stay on the safest path.}
%     % \vspace{-13pt}
%     \vspace{-5mm}
%     \label{fig:realworld}
% \end{figure}



\subsection{Ablation Studies}

\noindent\textbf{Effect of Multi-scale Fusion Design:} In Table~\ref{tab:ablation3}, we show the effect of our multi-scale fusion design with group-wise attention. We show an improvement of $14.76\%$ and $11.43\%$ in terms of mIoU on RUGD and RELLIS-3D, respectively.


\noindent\textbf{Group-wise Attention (GA) Design:} In Table~\ref{tab:ablation}, we show the effect of our segmentation head design with different backbones on both the RUGD and RELLIS-3D datasets. 
% We observe that, regardless of the backbone choice, group-wise attention improves performance (in terms of mIoU) by $7.26-11.44\%$ and $4.18-10.31\%$ on RUGD and RELLIS-3D, respectively. 
We observe that, regardless of the backbone choice, group-wise attention improves performance (in terms of mIoU) by $7.26-11.44\%$ on RUGD. 


\begin{figure*}[t]
    \centering

    \begin{subfigure}[c]{0.95\textwidth}
    \includegraphics[width = \textwidth]{fig/navigation_results_updated.png}
    \end{subfigure}

    \caption{\textbf{Navigation Results:} Trajectories when navigating with Ours (red), Segformer (orange), OCRNet (yellow), and DWA (green). (a) Walkway (concrete); (b) Trail (concrete with dirt and stone); (c) Dirt and grassy road; (d) Off-road. We observe that the trajectories generated by \ours{} maximize navigation along the smoothest surface of available terrains while maintaining the highest success rate.}
    \label{fig:navigation_reuslts}
    \vspace{-6mm}

\end{figure*}


\noindent\textbf{Ablation on Spatial Reduction with GA Head:} In Table~\ref{tab:ablation2}, we show the relations between performance and resolution change during spatial alignment. We can see that without GA heads, as we change the resolution to 1/16 and 1/32, there are performance drops of $1.3\%$ and $4.0\%$ in terms of mIoU on RELLIS-3D. 
% The performance drops do not appear for RUGD when we change the spatial reduction from 1/8 to 1/16; the main reason may be that the overall performance is low for RUGD before using GA heads, or the original resolution for RUGD is lower than RELLIS-3D, so the performance drop due to spatial information loss has not started to appear. We can still see the performance drop when reducing it to 1/32. 
After we add the GA component, the mIoU performance improves by $2.85-5.85\%$ on RELLIS-3D. In addition, we no longer see the performance drop on RELLIS-3D with the proposed GA heads. Use of GA heads allows us to reduce spatial resolution for efficient inference without compromising the final performance.



% \subsection{Qualitative Results}

% In Fig~\ref{fig:visualisations}, we show some visual results of \ours{} and two other state-of-the-art segmentation methods. 






\subsection{Improved Outdoor Navigation using \ours{}}
\label{nav_comparisons}



We evaluate the benefits of our \ours{} segmentation algorithm for robot navigation in real-world outdoor scenarios using a Clearpath Jackal and a Husky robot mounted with an Intel RealSense camera. The camera has a field of view (FOV) of 70 degrees. We use an Alienware laptop with an Intel i9 CPU (2.90GHz x 12) and an Nvidia GeForce RTX 2080 GPU mounted on the robot to run \ours{}.
% at a rate of 12Hz. 
We also utilize a velodyne 3D Lidar for robot localization and elevation map generation. 
%the robot for the DWA~\cite{dwa} planner. 
We test the navigation performance of our segmentation and elevation-based planner on a variety of terrains around a university campus, including concrete walkways, asphalt trails, dirt roads, and off-road terrains. 
%As shown in Figure~\ref{fig:realworld}, our method can correctly identify different regions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We have a pitch of 15-20 degree towards the ground, and camera height is 0.25-0.3m.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We apply DWA~\cite{dwa} to plan trajectories for the robot to reach a user-defined goal. The navigation stops when there is no viable trajectory based on the perception result. We test our method on six different routes, and the navigation results are shown in Table~\ref{tab:perf}. 

% Our method is very robust to new unstructured environments and can safely reach the goal five out of six times, while other methods cannot reach the goal most of the time. We also exceed other methods in average progress towards goal by 54.73\% and reduce the false positive rate of forbidden regions by 29.96\%.

% The only case that our method failed is when \ours{} misclassify a brick road as obstacles.

%\subsection{Evaluation Metrics for Navigation}

The following metrics are used to compare the navigation performance of our method with the Dynamic Window Approach (DWA)~\cite{dwa}, TERP~\cite{terp}, Segformer~\cite{segformer}, and OCRNet~\cite{yuan2020objectcontextual} based planners.

\begin{itemize}
\item \textbf{Success Rate: } The number of successful attempts for the robot to reach its goal while avoiding non-traversable regions and collisions over the total number of trials.

\item \textbf{Trajectory Roughness:} The cumulative vertical motion gradient experienced by the robot along a trajectory.


\item \textbf{Trajectory Selection:} The percentage of the robot's trajectory length along the most navigable surface out of the total trajectory length (i.e., the selection of smoother regions over others).


\item \textbf{False Positive of the Forbidden Region:} The percent-age of the frames that include a misclassified forbidden region out of all the frames during navigation.


\end{itemize}




\input{Tables/realworld_perf}



% \subsection{Navigation Comparisons}
% The navigation results 
% for \ours{}, DWA~\cite{dwa}, TERP~\cite{terp}, Segformer~\cite{segformer}, and OCRNet~\cite{yuan2020objectcontextual} based planners 
% are shown in Table \ref{tab:comparison_table}. 
In Table~\ref{tab:comparison_table}, we observe that all three segmentation-based planners perform well in terms of success rate under Walkway and Trail scenarios due to the clear margins between the different surfaces (see Fig. \ref{fig:navigation_reuslts}(a) and  \ref{fig:navigation_reuslts}(b)). Even though Segformer~\cite{segformer} and OCRNet~\cite{yuan2020objectcontextual} exhibit reasonable performances under scenarios similar to trained datasets, we observe significant performance degradation in terms of trajectory selection during off-road conditions.  However, \ours{} results in significant improvements in terms of all four metrics in cluttered and unseen scenarios such as Dirt-road and Off-road. Especially, accurate segmentation from \ours{} increases the utilization of the most navigable surface during planning as shown in Fig. \ref{fig:navigation_reuslts}(c) and  \ref{fig:navigation_reuslts}(d). This improved segmentation leads to better trajectory selection performance than the other methods, as shown in Table \ref{tab:comparison_table}. 

% \textbf{Elevation Only vs Elevation with Segmentation:} 
Our baseline planner TERP only incorporates terrain elevation data to perform the navigation task. Hence, it cannot differentiate surface characteristics in multi-terrain scenarios with similar elevations. This leads to trajectory generation along less navigable surfaces. Therefore, we observe a noticeable degradation in terms of trajectory smoothness in TERP~\cite{terp}. However, the utilization of semantic segmentation data from \ours{} for the baseline planner significantly enhances the navigable trajectory selection capabilities of the algorithm. 

==> sections/overview.tex <==
\section{\ours{} For Terrain Classification}
% Based on the navigability levels defined in the previous section, we transform the labels in the RUGD and RELLIS-3D datasets into 6 classes for semantic segmentation. 
% % As reported by RUGD \cite{RUGD2019IROS} and RELLIS-3D\cite{rellis}, most current state-of-the-art segmentation methods do not work well on the 24 class setting. 
% While a naive re-labeling helps increase the accuracy, we show that we can significantly improve the performance using a new transformer network specifically designed to take advantage of class groupings via group-wise attention.
% % While the relabeling scheme results in a considerable improvement in accuracy, we show that a careful design of architecture that leverages this grouping scheme can further improve performance. In addition, before the relabeling step, we create a new train-validation-testing set that distributes the classes uniformly. 

% MOD
% We present \tian{TBD}- a bottleneck transformer-based semantic segmentation network for navigation in off-road terrain. As shown in Figure \ref{fig:overview}, our architecture consists of a transformer backbone, and leverages multi-class self attention to focus on the various categories. In addition to optimizing using the direct branch, we propose a group wise attention loss to guide the network towards individually segmenting the various groups. The rest of this section is structured as follows. We formally define our problem in section \ref{def}, and the backbone architecture in section \ref{transnet}. Our architecture, which builds on multi-head self-attention is detailed in section \ref{TGAhead}, and the optimization cost functions are explained in section \ref{loss}. 




We present \ours, an approach for classifying the navigability of different terrains in off-road environments via coarse-grained segmentation.
Most of the existing segmentation methods fail in unstructured environments due to highly similar visual features and unclear boundary of the objects.
Use of multi-head self-attention is popular in neural network design due to its superior performance over prior state-of-the-art methods in segmentation~\cite{setr, dpt}, image classification~\cite{pham2021meta}, and object detection~\cite{coco, srinivas2021bottleneck, m3detr}, but the quadratic nature of its computational complexity has been an issue for real-time use like navigation.

To solve performance degradation in unstructured environment and computation limitation, we design a simple and lightweight architecture, which uses self-attention at the multi-scale fusion step and generated attention maps to calculate loss for better performance and low level of computational overhead.

% Considering the run-time requirement for navigation, we design a simple and lightweight structure, which uses self-attention at the multi-scale fusion step, and use generated attention maps to calculate loss for better performance and less computational overhead.
% \tian{Note: We also remove the attention branch during inference time for computation efficiency and fast run-time. }

% We also remove the attention branch during inference time for computation efficiency and fast run-time.

% To address the limitations of long-tailed distributions of terrain classes in such environments, our method leverages group segmentation via a group-wise attention mechanism. Our mechanism is a combination of group-wise attention heads and a novel attention loss function. 
% % In addition, we introduce a dynamically weighted cross-entropy loss function that can alleviate the long-tailed distribution issue via the notion of class weights. 
% Our approach is general and can handle dynamic groupings depending on the robot hardware and terrain classes.

% For the rest of this section, we will discuss the problem statement, various components of \ours{}, different between our method and other attention-based methods, and briefly explain its integration with planning and navigation.

% The rest of this section is structured as follows. We begin by stating our problem in Section~\ref{def}. We then discuss the various components of our approach, namely the backbone architecture (Section~\ref{backbone}), \ours{} segmentation head (Section~\ref{group_wise}), and an attention-based loss function (Section~\ref{loss}). Finally, we clarify the difference between \ours{} and other attention-based methods and briefly explain our integration with planning and navigation module for navigation demonstration.


% and we move on to our post-grouping strategy and explain the choice of the backbone in our segmentation networks in \ref{transnet}. We formally present our proposed detection head and details of motivations for the proposed group-wise attention in section \ref{group_wise}.
% the backbone architecture in section \ref{transnet}. Our architecture, which builds on multi-head self-attention is detailed in section \ref{TGAhead}, and 
% Finally, the optimization cost functions are explained in section \ref{loss}.


% general and flexible framework of determining navigability based on semantic segmentation network for reliable navigation in off-road terrain. Based on the grouping discussed in section \ref{groupings}, we proposed a post-grouping method that levitate the issue of long tail distribution in training data. We discover that our grouping scheme has improvement over existing methods in terms of error rate on the groups, and our proposed network can achieve state-of-the-art performance on existing off-road dataset. Our approaches effective solve the long-tail problem by shifting complex semantics to groups that are relevant for the navigation task, particularly in unstructured outdoor environment. 



\subsection{Problem Definition}
\label{def}
The input consists of an RGB image $I \in \mathbb{R}^{3\times H \times W}$ and the corresponding ground-truth semantic segmentation labels $Y\in \mathbb{Z}^{H\times W}$ denoting the category to which each pixel belongs among $G$ different groups. We use new coarse-grain labels $Y_G \in \mathbb{Z}^{H\times W}$ based on sematic labels provided by the dataset. For each group, we also compute the binary mask $Y_{B_g} \in \{0, 1\}^{H\times W}$ for $g = 1, ..., G$. Our goal is to perform coarse-grain semantic segmentation on terrain images $I$ and compute probability maps $P\in\mathbb{R}^{G\times H \times W}$. Each entry in $P$ is a probability distribution of a pixel in that entry location belonging to one of the $G$ groups.  
% $G$ could be dependent on the nature of the task; for example, an off-road navigation task should have more fine-grained classes on different types of roads. In contrast, in the context of collision avoidance, the focus should be on different kinds of obstacles for location and moving capabilities.



% \begin{figure}[t]
%     \centering
%     \includegraphics[width = \columnwidth]{fig/backbone.png}
%     \vspace{-15pt}
%     \caption{A selection of the backbones: \textbf{Top:} A representation of the ResNet-50. \textbf{Bottom:} A representation of the Bottleneck Transformer\cite{srinivas2021bottleneck}. In \cite{srinivas2021bottleneck}, they use Multi-Head Self-Attention (MHSA) to replace a 3x3 convolution operation during the last stage. Note that we ignore the initial 7x7 convolution, ReLU and 2D max pooling layer in the representation. And we also ignore the the 2D batch normalization after each block except the ReLU block. }
%     \vspace{-10pt}
%     \label{fig:backbone}
% \end{figure}

% \subsection{Data Pre-processing}


\subsection{Backbone Design}
\label{backbone}
% \subsection{Post-grouping Solution: Transformer Backbone}


% In prior semantic segmentation approaches for off-road terrains, the ResNet-50 and ResNet-101 were the primary choice for the architecture of the deep neural network (DNN). Recently it has been shown that Transformers~\cite{attentionisallyouneed} consistently outperform the ResNet family of architectures on several tasks including object detection~\cite{detr}, image classification and semantic segmentaion~\cite{srinivas2021bottleneck, cao2019gcnet}. 


% \rohan{Rephrase the below text to focus on why and how you use MHSA for group-wise attention-based segmentation.}
% In Figure \ref{fig:backbone}, we layout our implementation of the Bottleneck Transformer and highlight the differences. In summary, the Bottleneck transformer modifies the last stage of ResNet-50 and replaces the corresponding 3x3 convolution layer with a Multi-Head Self-Attention layer (MHSA). %In general, Bottleneck Transformer shows better learning results than ResNet-50, as demonstrated in \ref{exp}.

% \subsection{Group-wise Attention Head}
% \label{TGAhead}

% To explicitly guide individual group predictions, we propose leveraging multi-head self attention. Multi-head self attention constructs multiple representation subspaces by using multiple blocks of self-attention, which perseveres to capture regions of the scene to `focus' on or `attend' to. We now describe the notion of multi-head self-attention, which needs an understanding of self-attention. 

% \paragraph{Self-attention:} Consider two input matrices $X_L \in \mathbb{R}^{L\times D_{in}}$ and $X_S \in \mathbb{R}^{S\times D_{in}}$, where $L$ and $S$ are the lengths of the input sequence of $D_{in}$. The attention layer output is defined as:\vspace{-5 pt}

% $$\textrm{Attention}(Q, V, K) = \textrm{Softmax}(\frac{QK^{T}}{\sqrt{D_{in}}})V \in \mathbb{R}^{L\times D_{out}},$$ 
% $$\textrm{where}\  Q = X_LW_Q,\  K = X_LW_K\  and\  V = X_SW_V.$$

% The matrices $Q$, $K$ and $V$ represent query, key and value respectively, obtained by projection matrices $W_Q, W_K\in \mathbb{R}^{D_{in}\times D_{h}}$ and $W_V\in \mathbb{R}^{D_{in}\times D_{out}}$, where $D_{h}$ is the hidden dimension. The attention map $A$ is defined as:

% $$A = \textrm{Softmax}(\frac{QK^{T}}{\sqrt{D_{in}}}) \in \mathbb{R}^{L\times L}$$

% When two input matrices $X_L$ and $X_S$ represent the same feature maps, the attention module is usually referred to as self-attention. 

Vision Transformers (ViTs)~\cite{srinivas2021bottleneck, 16x16} are a type of deep neural network (DNN) for feature extraction and are designed as an alternative to the widely used ResNet~\cite{resnet} architecture via Multi-Head Self-Attention (MHSA). MHSA, or self-attention applied on image patches, is the main component of ViTs, contributing to much of their success over ResNets in computer vision-based tasks. Our approach also uses a transformer-based backbone architecture and leverages the MHSA module to extract and fuse multi-scale features. Our architecture can adapt to any backbone design with multi-scale features; in particular, we use Mixed Transformer (MiT)~\cite{segformer} with some modifications as our backbone. In addition, to show the advantages of our design, we also show two alternative backbones with our design, ResNet50~\cite{resnet} and Bottleneck Transformer (BoT)~\cite{srinivas2021bottleneck}.

Given an RGB image $I \in \mathbb{R}^{3\times H \times W}$, we first divide it into several patches as input to the transformer encoders. Unlike ViT and MiT, which take non-overlapping patches of shape 16 by 16 and 4 by 4, respectively, we choose patches of size 7 by 7 with a stride of 4 in our design. After passing the patches to the first transformer encoder blocks, we continue to take 2 by 2 patches on the output features. Therefore, after the initial encoders, each following block of transformer encoders reduces the spatial resolution further by a factor of 2 on both height and width. After each transformer encoder block, we obtain multi-scale features $F_i$ with spatial resolution $H_i \times W_i = \frac{H}{2^{i+1}} \times \frac{W}{2^{i+1}}$, where the feature channel $C_i$ = \{32, 64, 160, 256\} and i = \{1, 2, 3, 4\}. We utilize all multi-scale features in our segmentation head.

% \subsection{Multi-scale Feature Fusion with Group-wise Attention}
\subsection{\ours{} Segmentation Head}
\label{group_wise}

We introduce our novel group-wise attention (GA) heads for multi-scale features fusion. Our design can boost the performance on different backbone designs and mitigate the performance drop caused by resolution reduction mentioned below.
In previous step, the RGB image $I$ is passed through the feature extractor to obtain multi-scale feature maps $F_i \in \mathbb{R}^{C_i\times H_i \times W_i}$ after $i$-th encoder block. 

\noindent\textbf{Spatial Alignment and Resolution Reduction:}
In order to perform multi-scale features fusion, we need to combine features at the same spatial locality. We use bi-linear interpolation to resize $F_i$ into shape ($C_i\times H_f \times W_f$), where $H_f$ and $W_f$ are equal to $H_i$ and $W_i$ with a chosen $i$ among all scales. The final feature before fusion, $F_{fuse}$, is concatenated over channel dimension with shape ($\sum{C_i}\times H_f \times W_f$)). 

To reduce the computational complexity, our efficient design prefers to align patch features from different scales to one scale with a smaller spatial resolution as the network bottleneck (i.e., choose a smaller $H_f$ and $W_f$). As we expect, as we reduce $H_f$ and $W_f$, the spatial resolution of $F_{fuse}$ reduces so the complexity goes down with some performance degradation. In Section~\ref{loss}, we also introduce the group-wise attention loss to not only improve the overall performance but also mitigate the performance drop from choosing a smaller spatial resolution. 

\noindent\textbf{Multi-scale Fusion with Group-wise Attention:}
Given an input feature vector $A_{in} \in \mathbb{R}^{N\times C_{in}}$, the output self-attention map $A_{out}\in \mathbb{R}^{N\times C_{out}}$ is computed as follows:
\begin{equation}
     A_{out} = softmax(k(A_{in})^T \cdot q(A_{in}))^T \cdot v(A_{in}),
     \label{eq: attention}
\end{equation}
% $$A_{out} = softmax(k(A_{in})^T \bigodot q(A_{in}))^T \bigodot v(A_{in})$$, 
where $k(A_{in}),\ q(A_{in}),\ v(A_{in})$ represent the key, query, and value feature maps, respectively, and $k$, $q$, $v$ are linear projections, as in the self-attention \cite{attentionisallyouneed} literature. 

This feature map $F_{fuse}$ is reshaped (and transposed) into $F_{flat} \in \mathbb{R}^{ H_fW_f\times \sum C_{i}}$, which is passed through the MHSA block with $G$ attention heads. The MHSA component fuses flatten multi-scale feature $F_{flat}$ to produce the new feature maps $F_{out} \in \mathbb{R}^{C_{out}\times H_f \times W_f}$ and generates $G$ attention maps (one for each group), $A_1, A_2, \ldots, A_G \in[0, 1]^{H_f W_f\times H_f W_f}$. The final output $P\in\mathbb{R}^{G\times H \times W}$ is obtained through a standard procedure of a segmentation network by a series of $1\times1$ convolutions and up-sampling from $F_{out}$. 


% has been proven to be a strong component of the feature extractor in computer vision problem. It can selectively attend to important features and adjust features multiple time by connecting several layers. In such exploration, it has been used in the backbone of DNN for feature extraction and \cite{srinivas2021bottleneck} demonstrate such advantage in several tasks.

% We initially group all categories into $G$ groups and obtain $Y_G$. As shown in Figure \ref{fig:overview}, our architecture consists of a Bottleneck Transformer(BoT)~\cite{srinivas2021bottleneck} and multi-head self-attention (MHSA) to leverages multi-group self attention to focus on the various categories. 
% MHSA with $N$ heads and the input matrix $X$ is defined as follows: 

% \[\textrm{MultiHead}(Q, K, V) = \textrm{Concatenate} [\textrm{head}_1, ..., \textrm{head}_N] W ^O, \]

% \noindent where $ \textrm{head}_i = \textrm{Attention}(QW_{i}^{Q'}, KW_{i}^{K'}, VW_{i}^{V'})$ and $Q, K, V$ are linear projections of X. The projection matrices $W^{Q'}_i \in \mathbb{R}^{D_h\times d_{k}},\  W^{K'}_i \in \mathbb{R}^{D_h\times d_{k}},\  W^{V'}_i \in \mathbb{R}^{D_h\times d_{v}},\  W^O \in \mathbb{R}^{Nd_v\times d_{out}}$ are learnable parameters in the network that correspond to each of the attention heads, where $d_k$ and $d_v$ are the hidden dimensions of each attention head for $K$ and $V$ respectively. Through Multi-Head Self-Attention operation, we can also obtain a set of self-attention maps $A$ of length $N$ where: 

% \[A_{i} = Softmax(\frac{QK^{T}}{\sqrt{D_{in}}}) \in [{0,1}]^{L\times L}.\]

% \noindent Let feature matrix $F \in \mathbb{R}^{D_{in}\times H_f \times W_f} $ be the output of the segmentation backbone and $G$ be the number of groups that we want to predict.
% The feature map $F$ is reshaped (and transpositioned) into $F_{flat} \in \mathbb{R}^{ H_fW_f\times D_{in}}$, which is passed through the MHSA block with $G$ attention heads to obtain the output feature maps $F'_{out} \in \mathbb{R}^{ H_fW_f\times D_{in}}$, reshaping which gives us $F_{out} \in \mathbb{R}^{D_{out}\times H_f \times W_f}$. The final output $P\in\mathbb{R}^{G\times H \times W}$ is obtained through a series of $1\times1$ convolutions and upsampling. In the next section, we will talk about our proposed detection head.




% \subsubsection{Attention Heads}

As demonstrated in Fig.~\ref{fig:overview}, in our detection head, we use MHSA to fuse multi-scale features and generate different attention maps for each group. We use those attention maps as an additional branch in the detection head and train the detection head to resemble the group distribution by explicitly guiding each attention map towards a corresponding category using a binary cross-entropy loss. Our network skips the attention map processing branch during inference time for efficiency.
% Attention maps can also capture the relevancy between two pixel locations. Intuitively, $A_{g, [x, y]}$ represents the amount of attention that the pixel at the $x^\textrm{th}$ position must pay to the pixel at the $y^\textrm{th}$ position. Given an attention map $A_g$, its main diagonal represents the relevance of each location with respect to the attention head $h_g$. We train the attention network to learn feature maps that are most relevant to its corresponding group through group-wise attention loss.
Our novel design of group-wise attention for multi-scale fusion can outperform existing transformer-based methods with outstanding efficiency on coarse-grain segmentation tasks in challenging off-road environments.

% Attention networks thus strive to learn feature maps that emphasize the relevance between a pair of locations, i.e., locations with high relevance have a high softmax score and vice versa.

%In the context of image processing, we have $L = H\times W$. 
% Attention maps can provide co-relational information between two pixel locations, and the main diagonal of $A_i$ represents the relevance of each location with respect to the attention head $h_i$. 

% The error will propagate through the network to the projection matrix used to generate $Q$ and $V$. Group-wise attention will guide the network towards individually segmenting the various groups. Note that our methods is specifically designed for segmentation with few categories, as more categories will require more attention heads. In multi-head self-attention, as the number of heads increases, the GPU memory will explore; therefore, it did not generalize well with too many categories.

% Intuitively, $A_{i, [x, y]}$ represents the importance of the feature at the $y$-th location with respect to the feature at the $x$-th location, i.e. it quantifies the amount of attention that the pixel at $x$-th position needs to pay to the pixel at the $y$-th position. Training boosts up the attention score when two locations are highly relevant. %In the context of image processing, we have $L = H\times W$. 
% Attention maps can provide co-relational information between two pixel locations, and the main diagonal of $A_i$ represents the relevance of each location with respect to the attention head $h_i$. 


%In addition, we obtain auxiliary outputs $A^{out}_i \in \mathbb{R}^{H \times W}$ for each group from the attention maps $A^{map}_i \in\mathbb{R}^{H_f W_f\times H_f W_f}$ for an auxiliary loss term as defined below \divya{Can we provide some intuition here?}. 


%we can also obtain list of attention maps $A^{maps}$ of length $G$, where each . By taking the main diagonal of $A^{map}_i$, reshaping and up-sampling, we can also obtain  as an auxiliary output for calculating loss and back-propagation. Each elements in $A^{out}$ corresponds to one group in our definition.




\subsection{Group-wise Attention Loss}
\label{loss}

Whenever we choose to reduce the resolution during the spatial alignment step, performance degradation is unavoidable. Based on the structure of our group-wise attention head, we propose group-wise attention loss to improve the performance and mitigate such effects. 

For each attention head $h_i$, we have its corresponding attention map $A_i \in [{0,1}]^{L\times L}$, where $L = H_f\times W_f$. We take the main diagonal of $A_i$ and reshape it to $B_i \in [{0,1}]^{H\times W}$ using bi-linear image resizing. Each pixel in $B_i$ represents the self-attention score with respect to $h_i$.
 
To guide each attention-map in the multi-head self-attention module, we apply a binary cross-entropy loss function: 
\begin{equation}
     \mathcal{L}_{\textrm{GA}}^{g} = - \sum_{h,w} y_{\textrm{G}} \log(B_g),
     \label{eq: loss_cA}
\end{equation}
where $y_G \in Y_G$. This equation calculates the loss between the predictions of the self-attention output and the corresponding group's binary ground truth with respect to the group. 

% The purpose of group-wise attention loss is not to use attention maps to accurately predict the group's distribution; instead, as an intermediate layer, it aims to provide guidance regarding which region an attention head should focus on for further classification.

As in traditional segmentation models, we optimize our network with a multi-class cross-entropy loss and an auxiliary loss:

\noindent\textbf{Cross-Entropy Loss:} This is the standard semantic segmentation cross-entropy loss, defined as follows:
\begin{equation}
     \mathcal{L}_\textrm{CE} = - \sum_{h,w} \sum_{g\in G
     } y_\textrm{GT}\log(P_g
     ),
     \label{eq: loss_ce}
\end{equation}
where $h,w$ represent the dimensions of the image, $G$ represents the set of groups, $P_g$ denotes the output probability map corresponding to group $g$, and $y_{GT}$ corresponds to the ground-truth annotations.


% \noindent\textbf{Group-Wise Attention Loss:} To guide each attention-map in the multi-head self-attention module, we apply a binary cross-entropy loss function (equation \ref{eq: loss_ce}) between the predictions of the self-attention output and the corresponding group's binary ground truth. The purpose of group-wise attention loss is not using attention maps to accurately predict the groups distribution; instead, as an intermediate layer, it aims to provide guidance on which region an attention head should focus on for further classification.
%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{equation}
%      \mathcal{L} = \mathcal{L}_{\textrm{CE}} + \sum_{g\in G} \mathcal{L}_{\textrm{GA}}^{g}
%      \label{eq: loss_cA}
% \end{equation}


% \begin{equation}
%      \mathcal{L}_{\textrm{GA}}^{g} = - \sum_{h,w} y \log(B_g)
%      \label{eq: loss_cA}
% \end{equation}



% \begin{equation}
%      \mathcal{L}_\textrm{CE} = - \sum_{h,w} \sum_{g\in G
%      } y\log(P_g)
%      \label{eq: loss_ce}
% \end{equation}

% \noindent $h,w$ -- the dimensions of the image.

% \noindent $G$ -- the set of groups.

% \noindent $P_g$ -- the output probability map corresponding to group $g$.

% \noindent $y$ -- 0/1 encoding of the ground-truth groups.

% \noindent $B_g$ -- the main diagonal of $A_g\in [{0,1}]^{hw\times hw}$, the corresponding attention map generated from attention head $h_i$.

% \noindent $y$ -- 0/1 encoding of the ground-truth groups.

%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent\textbf{Auxiliary Loss via Deep Supervision:} Deep supervision was first proposed in \cite{deepsuper} and has been widely used in the task of segmentation \cite{zhao2017pyramid, yuan2020objectcontextual}. Adding an existing good-performing segmentation decoder head like FCN~\cite{long2015fully} in parallel to our GA head during training not only provides strong regularization but also reduces training time of \ours{}. 


% \subsection{Dynamic weighting}
% \label{dw}
% Models trained on datasets with long-tailed distribution of classes can be biased towards the most frequent classes. There are  many techniques~\cite{zhang2018generalized, cui2019classbalanced} to re-weight classes or effective samples to deal with label corruption and long-tail distribution by giving priority to rare classes. To assist the model in learning feature representations for all classes uniformly, we adapt a weighted cross-entropy loss function in which the weights are determined by a new dynamic weighting strategy based on class error rate.% which is proven to be useful in Section~\ref{exp}. 

% Let the weights at the first epoch be $W_{init} \in \mathbb{R}^G$ and the weights at the $i^{th}$ epoch be $W_{i} \in \mathbb{R}^G$. After $d$ more epochs, the weight update rule is given as: 

% \begin{equation}
%      \mathcal{W}_{i+d} = m * W_{i} + (1 - m) * (W_{init} + W^d_{error}),
%      \label{eq: dw_equation}
% \end{equation}
% where $m$ is the momentum and $W^d_{error}\in[0, 1]^G$ is the error rate of each group during the intermediate $d$ epochs. 

% The momentum term assures that the change in weights is not drastic. Thus, the dynamic weighting scheme increments the weights in small steps. Additionally, our method can adaptively assign weights in accordance with the stage of training. The usage of the initial weights in the second term prevents bias towards a specific class. %using the initial weighting from the second term.% 
% Our dynamic weighting scheme aims to make small adjustment based on the initial weighting from the hyper-parameters. With dynamic weight, we achieve an improvement of 3.76\% in mean accuracy for RELLIS-3D dataset.

% \subsection{Difference between Existing Methods and \ours{}}
\subsection{ \ours{} v.s. Prior Segmentation Methods}

We compare and highlight some differences between \ours{} and prior transformer-based segmentation methods. 

SETR~\cite{setr}, DPT~\cite{dpt}: The designs are significantly different, particularly in terms of the computational overhead of those methods. In addition, these methods use positional embedding in the encoding stage, while our method removes any positional embedding in the backbone.

Segformer~\cite{segformer}, Segmenter~\cite{segmenter}: Those methods, as well as \ours{}, also focus on efficient training and inference. Segformer does not have any parameters dedicated to different classes except for the final classification layer. In addition, the decoder consists of several MLP layers for simple and efficient design. Segmenter and \ours{} both have trainable parameters dedicated to specific classes/groups: Segmenter uses $G$ class embeddings that correspond to each semantic class and appends those tokens to the end of the entire image patch sequence for the decoder, while \ours{} splits feature channels into $G$ portions of equal size for different attention heads that belong to different groups. Finally, \ours{} uses a smaller spatial resolution in the decoder bottleneck than the other two methods to improve the run-time and compensated for the complexity brought by MHSA.



\subsection{\ours{}-based Segmentation for Robot Navigation}
We combine \ours{} with TERP~\cite{terp}, an outdoor navigation planner to highlight the benefits of our segmentation algorithm for robot navigation. TERP utilizes the robot's pose, goal information and a point cloud based elevation map to generate a cost map from an attention based perception module. Before interfacing with TERP, we convert \ours{}'s segmentation results into a segmentation cost map. This is performed based on the following steps: 1. Projecting \ours{}'s segmented output onto the ground plane in front of the robot using homography transformations, and 2. Assigning discrete cost values for the different groups. We assign zero cost for smooth regions and increase the non-zero costs for rough, bumpy, forbidden and obstacle regions. 

The computed segmentation cost map is element-wise added with the elevation cost map generated from TERP's perception module to obtain the final navigation cost map. This resulting cost map is fed into TERP's navigation module, which computes least-cost trajectories towards the robot's goal. The overall system architecture is highlighted in Fig. \ref{fig:system-architecture}.

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{fig/system_architecture.png}
    % \vspace{-3mm}
    \caption{\textbf{\ours{}-Based Outdoor Navigation:} We integrate \ours{} with an elevation based planner TERP \cite{terp} to highlight benefits of our segmentation algorithm. Our architecture decouples semantic segmentation and elevation data for better perception and planning. The advantages of this formulation are highlighted in Section \ref{nav_comparisons}.}
    % \vspace{-13pt}
    % \vspace{-6mm}
    \label{fig:system-architecture}
\end{figure}






==> sections/related_work.tex <==
\section{Related work}
% We give a brief overview of prior work on robot navigation, semantic segmentation, and outdoor datasets.

\subsection{Semantic Segmentation}
Semantic segmentation is an important task in computer vision that involves assigning a label to each pixel in an image. The problem has been widely studied in the literature~\cite{hao2020brief}.
Many deep learning architectures have been proposed, including OCRNet~\cite{yuan2020objectcontextual}, PSPNet \cite{zhao2017pyramid}, etc. 
Most recently, there have been many transformer-based methods~\cite{setr, dpt, pvit, maskformer} that demonstrate better performance than other CNN-based methods but are computationally expensive. Therefore, there has been increased discussion of more efficient design based on transformers for fast inference time and lower computational cost, including \cite{segformer,segmenter}. 
While most of these architectures work well on structured datasets like CityScapes, they do not work well for off-road datasets due to ill-defined boundaries and confusing class features. 
% Segmentation methods like Global Convolution Networks \cite{peng2017large} are designed to deal with complex boundaries and do not scale well in terms of performance due to convoluted and overlapping boundaries that are generally not found in structured datasets.


\subsection{Navigation in Outdoor Scenes}
Prior work in uneven terrain navigation includes techniques for everything from mobile robots~\cite{outdoor, small_nav1, kahn2020badgr}
% \cite{outdoor, small_nav1, small_nav2, kahn2020badgr, robot_nav}
to large vehicles~\cite{large_nav1, off_road_trav1}. In these algorithms, learning the navigation characteristics of the terrain and its traversability is a crucial step. At a broad level, there are three types of approaches that are used to determine the terrain features: 1) proprioceptive-based methods, 2) geometric methods, and 3) appearance-based methods. The proprioceptive-based methods~\cite{vibrate1,vibrate2} 
% \cite{vibrate1,vibrate2,vibrate3} 
use frequency domain vibration information gathered by the robot sensors to classify the terrains using machine learning techniques. However, these methods require the robot to navigate through the region to collect data and assume that a mobile robot can navigate over the entire terrain. The geometric-based methods~\cite{off_road_trav1, roughness2}
% \cite{pointcloud_hazard, off_road_trav1, roughness1, roughness2}
generally use Lidar and stereo cameras to gather 3D point cloud and depth information of the environment. This information can be used to detect the elevation, slope, and roughness of the environment as well as obstacles in the surrounding area. Nevertheless, the accuracy of the detection outcome is usually governed by the range of the sensors. Appearance-based methods~\cite{sift_based} usually extract road features with SIFT or SURF features and use MLP to classify a set of terrain classes. 
% \cite{materials1, materials2} perform road material classifications. \cite{AdapNet} utilize deep neural network models for fine-grained semantic segmentation of urban scenarios to determine traversability of indoor scenarios. Additionally, there has been extensive work on the binary classification problem of segmenting roads into traversable or non-traversable regions~\cite{rural}.
% \cite{darpa, bigdog, rural, varma2018idd}
% Recently, \cite{} proposed context-aware navigation with some degree of terrain-awareness in less complicated outdoor environment.
Our goal is to focus on the visual perceptive, leveraging the performance and efficiency for robot navigation. Our method computes the navigable regions from RGB images in unstructured environments and outputs a safe trajectory in this condition.
% In this paper, we propose to segment the image on a comparatively fine-grained level to capture hard surfaces, obstacles, bumpy regions, etc which can be useful for a wide set of applications. %Overall, 




\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{fig/pipeline.png}
    \caption{\textbf{Architecture of our proposed network \ours:} 
    % We build on the transformer attention backbone \cite{segformer} and 
    We introduce a novel group-wise attention head for multi-scale fusion. After we convert multi-scale features into several groups of features, the group-wise attention loss acts between the multi-head attention outputs $A_g$ corresponding to group $g$ and the corresponding group-wise binary ground truth $Y_{B_g}$ to explicitly guide the network towards accurate predictions of different groups. 
    %In addition, we incorporate a dynamically weighted cross entropy-loss to handle the long-tailed nature of the dataset.
    }
    \label{fig:overview}
    \vspace{-15pt}
\end{figure*}

% \tian{OFFSEG~\cite{offseg} and OffRoadTranSeg~\cite{offtrans} are some recent segmentation methods proposed for unstructured environment and compete based on standard segmentation metric like mIoU. Our work performs coarse-grain segmentation based on traversability and aim to achieve good navigation result in off-road environment. }

\subsection{Off-road Datasets}
Recent developments in semantic segmentation have achieved high accuracy on object datasets like PASCAL VOC~\cite{pascal}, COCO~\cite{coco}, and ADE20K~\cite{ade20k2}, as well as driving datasets like Cityscape~\cite{cityscape}
% , CamVid~\cite{camvid}
and KITTI~\cite{kittiseg}. However, there has not been much work on recognition or segmentation in unstructured off-road scenes, which is important for navigation. Perception in an unstructured environment is more challenging since many object classes (e.g., puddles or asphalt) lack clear boundaries. RUGD~\cite{RUGD2019IROS} and RELLIS-3D~\cite{rellis} are two recent datasets available for off-road semantic segmentation. The RUGD dataset consists of various scenes like trails, creeks, parks, and villages with fine-grained semantic segmentation annotations. The RELLIS-3D dataset is derived from RUGD and includes unique terrains like puddles. In addition, RELLIS-3D includes Lidar data and 3D Lidar annotations. We use these datasets to evaluate the performance of our algorithm.






% \subsection{Transformer and Attention}
% Transformer was initially proposed in \cite{attentionisallyouneed} as an attention-based build block for deep model which takes a sequential input. Attention mechanism can selectively aggregate information from other part of the input sequence with different weight based on learned attention score. One main advantage of transformer is that they can take entire sequence at once, instead of relying on hidden state as memory in a sequence-to-sequence model like LSTM\cite{lstm}. It has been proven to be more stable in language translation than most auto-encoders, especially for long prediction sequence. 

% \tian{TODO}
% Due to the fact that transformer no longer requires a sequential input, there are been many recent works on feature extraction on both 3D point cloud data and 2D image as encoder. Currently, there is only one work that utilized 

